On the Workflows and Smells of Leaderboard Operations (LBOps): An Exploratory Study of Foundation Model Leaderboards

Foundation models (FM), such as large language models (LLMs), which are large-scale machine learning (ML) models, have demonstrated remarkable adaptability in various downstream software engineering (SE) tasks, such as code completion, code understanding, and software development. As a result, FM leaderboards have become essential tools for SE teams to compare and select the best third-party FMs for their specific products and purposes. However, the lack of standardized guidelines for FM evaluation and comparison threatens the transparency of FM leaderboards and limits stakeholders' ability to perform effective FM selection. As a first step towards addressing this challenge, our research focuses on understanding how these FM leaderboards operate in real-world scenarios ("leaderboard operations") and identifying potential pitfalls and areas for improvement ("leaderboard smells"). In this regard, we collect up to 1,045 FM leaderboards from five different sources: GitHub, Hugging Face Spaces, Papers With Code, spreadsheet and independent platform, to examine their documentation and engage in direct communication with leaderboard operators to understand their workflows. Through card sorting and negotiated agreement, we identify five distinct workflow patterns and develop a domain model that captures the key components and their interactions within these workflows. We then identify eight unique types of leaderboard smells in LBOps. By mitigating these smells, SE teams can improve transparency, accountability, and collaboration in current LBOps practices, fostering a more robust and responsible ecosystem for FM comparison and selection.

==> sections/10-authors-bio.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/ZhiminZhao.jpg}}]{Zhimin Zhao} is currently pursuing a PhD degree in the Software Analysis and Intelligence Lab (SAIL), Queen's University, Canada. He received his MSE degree from the SIG Center for Computer Graphics at the University of Pennsylvania, USA. His research interests include LLMOps, MLOps, and SE4AI. For more details on his work, visit https://zhimin-z.github.io.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/AbdulAliBangash.jpg}}]{Abdul Ali Bangash} is a Postdoctoral Fellow at Queen's University, Canada. He is privileged to be one of the six selected candidates who have been awarded the esteemed ``Vice-Principal Research (VPR) Postdoctoral Fund'' at Queen's University. He obtained his PhD in Computer Science from the University of Alberta, Canada, in 2023. His research interests include software engineering (SE) for AI (and vice versa), mining software repositories, search-based software engineering, and energy optimization. His work has been published in top software engineering venues such as ICSE, MSR, ICSME, and EMSE. He has served as a reviewer at renowned SE venues such as TOSEM, ICSE, MSR, and ICSME. For more details on his work, visit http://abdulali.github.io.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/FilipeRoseiroCogo.jpg}}]{Filipe Roseiro Côgo} is a software engineering researcher at the Center for Software Excellence of Huawei in Canada. His work focuses on the intersection of foundation models and software engineering, specifically in the areas of FM-powered software and SE-powered FMware. With a PhD from Queen's University, Filipe has extensive experience in applying machine learning and mining software repositories to investigate technical and social issues in software engineering. To learn more about his work, visit https://www.filipecogo.pro.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/BramAdams.jpg}}]{Bram Adams} is a full professor at Queen's University (up to June 2020: Polytechnique Montreal). He obtained his PhD in 2008 at Ghent University's GH-SEL laboratory (Belgium). His research interests include software release engineering, software engineering for artificial intelligence (AI) (and vice versa), and mining software repositories. His work received the Foundational Contribution Award for 2021 Mining Software Repositories. In addition to co-organizing the RELENG International Workshop on Release Engineering from 2013 to 2015 (and the 1st/2nd IEEE Software Special Issue on Release Engineering), he co-organized, amongst others, SEMLA 2018/19, FM+SE Vision 2030, and AIware 2024. He has been PC co-chair of SCAM 2013, SANER 2015, ICSME 2016, and MSR 2019; software analytics area co-chair of ICSE 2023, and general chair of MSR 2025. He is a Senior IEEE Member.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/AhmedEHassan.jpg}}]{Ahmed E. Hassan} is an ACM Fellow, IEEE Fellow, and NSERC Steacie Fellow. He is a laureate of the Mustafa Prize, a distinction equivalent in prestige to a Nobel, for founding the AI-augmented SE field and its associated Mining Software Repositories (MSR) conference. He is a Distinguished Educator of IEEE TCSE and an Influential Educator of ACM SIGSOFT. He is a recipient of the inaugural New Directions IEEE TCSE Award for his outstanding and sustained efforts to advance the field of AI-augmented SE. He is the Canada Research Chair (CRC) in Software Analytics and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen's University, Canada. For more details on his work, visit http://sail.cs.queensu.ca.
\end{IEEEbiography}

==> sections/discarded.tex <==
% ``test smells''~\cite{kim2020empirical}, ``security smells''~\cite{rahman2019seven}, ``data smells''~\cite{wu2023systematic}, and ``dependency smells''~\cite{jafari2021dependency}

% \section{Conflict of Interest}
% \label{sec:conflict}

% The authors declare that they have no conflict of interest.

%fan2023automated,qian2023communicative,gu2023llm,li2024enhancing,yang2024large

% \emph{Implication}: Unclear metrics could result in difficulties interpreting and comparing model performance. \\
% \emph{Implication}: Poor documentation of in-context learning configurations can cause inconsistent evaluation methods, compromising result reliability and comparability across ML models and studies. \\
% \emph{Implication}: Absent raw datasets can impede reproducibility, comparability, and transparency in ML model evaluations, causing potential inconsistencies in research outcomes. \\
% \emph{Implication}: Incomplete or inaccurate evaluation records can compromise reliable conclusions and model comparisons, potentially leading to misinformed decisions and research directions. \\
% \emph{Implication}: Inaccessible and inaccurate model information can impede result reproduction, relevance assessment, and informed decision-making regarding collaborations or model improvements in research. \\
% \emph{Implication}: Unclear ranking dataframes may cause user confusion, potentially leading to misinterpreted model rankings and inaccurate ML model performance evaluations. \\
% \emph{Implication}: Unclear submission guidelines can cause user confusion, leading to incorrect submissions, wasted resources, and a diminished user experience. \\
% \emph{Implication}: Deprecated benchmarks lead to potential user confusion, outdated evaluations, and resource misallocations in ML research. \\
% \hrule \noindent \\
% \emph{Component}: Evaluation Score \\
% \emph{Example}: Hundreds of evaluation records are deprecated for the ``junior-v1'' benchmark in the CanAiCode Leaderboard\footnote{\url{https://huggingface.co/spaces/mike-ravkine/can-ai-code-results/discussions/3}}. \\
% \emph{Implication}: Deprecated evaluations can confuse users about the leaderboard's reliability and relevance, potentially leading to misinformed decisions and research directions. \\
% \hrule \noindent \\
% \emph{Component}: Leaderboard Publication \\
% \emph{Example}: PromptBench had evolved considerably since its first release in \date{2023}, making the initial report deprecated\footnote{\url{https://github.com/microsoft/promptbench/issues/52}}\footnote{\url{https://github.com/microsoft/promptbench/issues/50}}. \\
% \emph{Implication}: Deprecated publications can cause incorrect assumptions, wasted time and resources, and misinformed research directions. \\
% \hrule \noindent \\
% \emph{Component}: Model \\
% \emph{Example}: There are dozens of deprecated models, such as ``OpenAI/text-davinci-001'', listed in the documentation of HELM Classic\footnote{\url{https://github.com/stanford-crfm/helm/issues/2386}}. \\
% \emph{Implication}: Deprecated models can mislead performance evaluation, confuse users, and increase the maintenance overhead of leaderboards. \\
% \emph{Implication}: Deprecated ranking dataframes can cause unreliable rankings, misinformed evaluations, and user confusion, compromising the integrity and usability of leaderboards. \\
% \hrule \noindent \\
% \emph{Component}: Submission Channel/Protocol \\
% \emph{Example}: The Spider leaderboard had deprecated its submission channels for an extended period due to ongoing maintenance issues\footnote{\url{https://github.com/taoyds/spider/issues/101}}. \\
% \emph{Implication}: Deprecated submission channels can restrict collaboration, delay updates, and reduce transparency, hindering progress in ML research. \\
% \emph{Implication}: Inaccessible benchmark datasets can hinder transparency, raise data integrity concerns, and limit user engagement, leading to imbalanced competition and potentially unreliable ML research. \\
% \emph{Implication}: Limited visibility of evaluation records may lead to a lack of transparency and trust in the leaderboard's fairness, potentially causing doubts about the leaderboard's ability to provide a comprehensive and unbiased evaluation of ML models. \\
% \hrule \noindent \\
% \emph{Component}: Leaderboard Publication \\
% \emph{Example}: The MathBench report was inaccessible from its project page\footnote{\url{https://github.com/open-compass/MathBench/issues/4}}. \\
% \emph{Implication}: Inaccessible publications can impede the spread of vital benchmarking information, limiting transparency and complicating researchers' efforts to comprehend evaluation methods, reproduce results, or advance previous work. \\
% \emph{Implication}: Limited model access in leaderboards can impede result reproducibility and comparability, decreasing the leaderboard's utility and potentially restricting collaboration and ML research progress. \\
% \emph{Implication}: Inaccessible ranking dataframes can hinder researchers' ability to evaluate ML models, affecting reliability and usability, and potentially slowing ML research progress. \\
% \emph{Implication}: Inaccessible submission channels can hinder collaboration and innovation, resulting in less diverse and potentially biased model evaluations. \\

% \emph{Implication}: Hidden or misdisplayed metrics can mislead ML model performance evaluation, causing researchers to invest in suboptimal models or solutions potentially. \\
% \emph{Implication}: Broken layout in benchmark protocol documentation can cause incorrect benchmark setups, unreliable results, and wasted resources in ML research. \\
% \emph{Implication}: Misrepresented ranking dataframes can confuse users about model performance, impacting leaderboard reliability and potentially leading to suboptimal ML research decisions. \\
% \emph{Implication}: Misrepresented ranking dataframes can confuse users about model performance, impacting leaderboard reliability and potentially leading to suboptimal ML research decisions. \\
% \emph{Implication}: Mismatched metrics may cause confusion, leading to inaccurate evaluations, misdirected ML research, and potential harm to the leaderboard's credibility. \\
% \emph{Implication}: Protocol discrepancies can cause misleading results, compromising the reliability of the leaderboard and potentially misguiding ML research efforts. \\
% \emph{Implication}: Mismatched datasets might lead to incomplete evaluations and potentially compromise the integrity of ML research.  \\
% \emph{Implication}: Mismatched task labels can mislead researchers by providing inaccurate task descriptions, potentially resulting in wasted resources and a lack of focus on the intended research objectives. \\
% \emph{Implication}: Inconsistent evaluation records can cause confusion and mistrust among users, potentially compromising the reliability and credibility of leaderboards and hindering the progress of ML research. \\
% \emph{Implication}: Inconsistent model specifications can cause confusion and misinformed decisions, potentially compromising the integrity of ML research and undermining trust in the leaderboards. \\
% \emph{Implication}: Mismatched ranking dataframes can confuse users and hinder accurate comparisons of ML model performance. \\
% \emph{Implication}: Missing protocol in benchmark documentation can cause inconsistent methodologies, compromising result reliability, and hindering accurate comparisons of ML models, potentially slowing the progress of research in the field. \\
% \emph{Implication}: Missing evaluation records can result in incomplete performance evaluation, potentially leading to suboptimal ML research decisions and slowing progress in the field. \\
% \emph{Implication}: Empty ranking dataframes can limit the availability of model performance information, hindering informed decision-making and potentially slowing progress in ML research.\\
% \emph{Implication}: Missing submission channels can limit collaboration and model contributions, potentially hindering leaderboard diversity and slowing progress in the development of advanced FMs. \\

% \emph{Implication}: Duplicate evaluation records can skew overall performance assessments, potentially leading to misinformed decisions and wasted resources in ML research. \\
% \emph{Implication}: Duplicate model names can cause ambiguity in model identification, potentially causing confusion, misinformed decisions, and hindering accurate performance comparisons in ML research. \\
% \emph{Implication}: Duplicate ranking dataframes can create unnecessary redundancy, diverting resources and attention from more critical aspects of ML research, such as model development and performance optimization. \\
%\emph{Implication}: Unresponsive ranking dataframes may lead to frustration among users, reduced credibility, and inefficient leaderboard management.\\
%\emph{Implication}: Unresponsive submission panels can impede users' ability to contribute models and compare performance, potentially hindering the growth of leaderboards. \\ 
% It extends to phrases such as ``exact match'', and ``exact match accuracy''\footnote{\url{https://paperswithcode.com/sota/text-to-sql-on-spider}}. Furthermore, there is a lack of clarity in differentiating terms such as ``accuracy'', ``average accuracy''\footnote{\url{https://paperswithcode.com/sota/video-question-answering-on-situated}}, and ``overall accuracy''\footnote{\url{https://rowanzellers.com/hellaswag}\label{footnote:HellaSwag}}. The terminology used in metrics, such as ``success rate''\footnote{\url{https://intercode-benchmark.github.io}\label{footnote:InterCode}}, ``win rate''\footref{footnote:AlpacaEval}, and ``pass rate''\footref{footnote:TravelPlanner}, often leads to confusion due to their overlap of definitions in various contexts. This issue is exacerbated in the PWC leaderboards, where various metrics related to specific papers are prone to being perceived as identical by users contributing new evaluation records, leading to increased user misinterpretation. 

%Finally, we present some leaderboard-related statistics to emphasize the prevalent characteristics relevant to leaderboard implementation.% Recognizing that requirement gathering, design, and deprecation are ubiquitous operations of any leaderboard, we have opted to exclude these phases from our analysis. Instead, we concentrate on the unique phases that distinguish the operationalization of these systems, emphasizing their specialized purposes and functionalities. 

% Furthermore, we observe that $93.89\%$ ($446/475$) of the leaderboards following $P_1$ are hosted on the PWC platform. In particular, $P_1$ is the only workflow pattern consistently used in all PWC leaderboards, highlighting its significance and widespread adoption within this platform. This is due to PWC's development of automated tools for collecting leaderboard data from academic articles\footref{footnote:axcell}, other leaderboards\footnote{\url{https://twitter.com/eval_ai/status/1341091250544521231}}, and model cards\footnote{\url{https://github.com/paperswithcode/model-index}\label{footnote:model index}}. 

% \subsection{Leaderboard Statistics}

% This section provides a comprehensive analysis of the distribution of key attributes in the leaderboards under investigation. These attributes include leaderboard publishers, leaderboard publications, and ranking dataframe display formats. By examining these aspects, we gain valuable insight into the characteristics and functionalities of various leaderboards, allowing for a better understanding of their roles within the broader context of model evaluation and ranking.

% \emph{Leaderboard publisher}: We find a high degree of inequality in the distribution of leaderboards among the $235$ identified organization. A Gini coefficient~\cite{gini1936measure}\footnote{Gini coefficient measures inequality, with values ranging from $0$ (representing perfect equality) to $1$ (denoting perfect inequality).} of $0.634$ indicates that a small number of organizations are responsible for operating multiple leaderboards, resulting in a concentration of control over releases. In particular, PWC stands out as the most prolific organization, contributing to notable $63.29\%$ ($443/1,045$) leaderboards. This is followed by AI2\footnote{\url{https://leaderboard.allenai.org}\label{footnote:AI2}} ($4.14\%$), Shanghai AI Laboratory\footnote{\url{https://www.shlab.org.cn}} ($3.86\%$), University of California\footnote{\url{https://www.universityofcalifornia.edu}} ($2.86\%$). Also, $3.86\%$ leaderboards are published by independent contributors not affiliated with any particular organization. The dominance of a few organizations in publishing leaderboards could lead to a concentration of influence over the direction and focus of research within the field. This might result in certain areas receiving more attention and resources, potentially at the expense of other important but less represented topics.

% \emph{Leaderboard publication}: We find that $85.2\%$ ($380/446$) of the leaderboards are associated with specific publications. Of these, $61.32\%$ ($233/378$) publications have been accepted in a specific workshop, conference, magazine, or journal, as opposed to being solely archived as arXiv reports or blog posts. The Gini coefficient of $0.647$ highlights substantial inequality in the distribution of leaderboards linked to various publication venues. In particular, EMNLP\footnote{\url{https://aclanthology.org/venues/emnlp}} stands out as the conference with the highest number of accepted publications, representing $16.74\%$ ($39/233$) of the total published. It is closely followed by NeurIPS\footnote{\url{https://neurips.cc}} ($10.73\%$), ACL\footnote{\url{https://aclanthology.org/venues/acl}} ($9.01\%$), and CVPR\footnote{\url{https://cvpr.thecvf.com}} ($8.15\%$). These statistics highlight that a significant portion of leaderboard-linked research is concentrated in a few high-profile venues, reflecting both the competitive nature and the recognized impact of these conferences and journals in the field.

% \emph{Ranking dataframe display format}: Ranking dataframes can be presented in various formats, including tables (\eg, regular table\footnote{\url{https://tatsu-lab.github.io/alpaca_eval}\label{footnote:AlpacaEval}}, rankable table\footnote{\url{https://huggingface.co/spaces/gsaivinay/open_llm_leaderboard}}, table screenshot\footnote{\url{https://github.com/MikeGu721/XiezhiBenchmark}\label{footnote:Xiezhi}}) or figures (\eg, bar chart\footnote{\url{https://leaderboard.tabbyml.com}\label{footnote:Coding LLMs Leaderboard}}, box plot\footnote{\url{https://artificialanalysis.ai/leaderboards/models}\label{footnote:Models Leaderboard}}, heat map\footnote{\url{https://github.com/Libr-AI/do-not-answer}\label{footnote:Do-Not-Answer}}, line chart\footnote{\url{https://xwang.dev/mint-bench}\label{footnote:MINT}}, pie chart\footnote{\url{https://osu-nlp-group.github.io/TravelPlanner}\label{footnote:TravelPlanner}}, radar chart\footnote{\url{https://huggingface.co/spaces/BramVanroy/open_dutch_llm_leaderboard}\label{footnote:Open Dutch LLM Evaluation Leaderboard}}, scatter plot\footnote{\url{https://huggingface.co/spaces/ml-energy/leaderboard}\label{footnote:ML.ENERGY Leaderboard}}, sortable bar chart\footnote{\url{https://huggingface.co/spaces/ramiroluo/LLMHallucination_Leaderboard}\label{footnote:LLMHallucination Leaderboard}}). Each format offers unique benefits for data visualization, enabling easy comparison or emphasizing critical performance insights. We find that $62.33\%$ ($278/446$) leaderboards support multiple display formats in their ranking dataframes. Furthermore, our analysis reveals that $76.68\%$ ($342/446$) leaderboards offer ad hoc ranking functionality, allowing users to interact with column names for personalized ranking and analysis. Among these, $99.71\%$ ($341/342$) utilize tables as the primary display format, with the sole exception of bar charts. Other less commonly used unrankable display formats include \textit{scatter plot} ($50\%$), \textit{regular table} ($26.68\%$), \textit{bar chart} ($6.95\%$), \textit{table screenshot} ($4.93\%$), \textit{radar chart} ($1.35\%$), \textit{line chart} ($0.45\%$), and \textit{heat map}, \textit{box plot}, and \textit{pie chart} both at $0.22\%$. These statistics underscore the importance of adaptable and versatile data visualization methods in presenting and comparing model performance on leaderboards.

% \emph{Leaderboard - storage format}: We find that only $12.98\%$ ($57/446$) leaderboards offer downloadable file formats for their leaderboards, allowing ML researchers to conduct more detailed investigations into model performance trade-offs. In particular, \textit{CSV} is the most prevalent downloadable storage format for leaderboards, accounting for $78.95\%$ ($45/57$) leaderboards. Other formats, including \textit{JSON} ($8.77\%$), \textit{XLSX} ($5.26\%$), \textit{TSV} ($3.51\%$), \textit{LATEX} ($3.51\%$), \textit{MD} ($1.75\%$), \textit{XLS} ($1.75\%$), and \textit{JSONL} ($1.75\%$), are less frequently used. 


% \subsection{Machine Learning Leaderboard Types}

% ML leaderboards are centralized software systems that enable stakeholders to evaluate and rank the performance of third-party ML models, algorithms, solutions, and even benchmark elements. Throughout the leaderboard collection (detailed in Section~\ref{sec:method:design}), we identify six unique types of ML leaderboards. Each type of leaderboard serves a unique ranking purpose, with the main difference being the specific element that each leaderboard evaluates. 
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Model-oriented leaderboards} focus on comparing FMs under a selective set of benchmarks. Representative examples are Chatbot Arena leaderboard and Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}, as shown in Figure~\ref{fig:leaderboard structure}. % By providing this information, these leaderboards allow researchers and practitioners to make informed decisions about model selection and optimization. 
%     \item \textbf{Dataset-oriented leaderboards} focus on comparing the efficacy of benchmark datasets under a selective set of metrics. Unlike traditional benchmarks that emphasize model architecture and hyperparameter tuning, for example, DataComp\footnote{\url{https://www.datacomp.ai/dclm/leaderboard.html}}%\footnote{\url{https://www.datacomp.ai/dcclip/leaderboard.html}} 
%     fixes the models and training code, allowing participants to create the most effective training datasets from a massive data pool. % By offering this information, these leaderboards allow researchers and practitioners to make informed decisions about dataset selection and optimization, ultimately leading to models being trained on the most effective data available.
%     \item \textbf{Metric-oriented leaderboards} focus on comparing evaluation metrics in a selective set of benchmarks under consistent model implementation. A representative example is the AlignScore leaderboard\footnote{\url{https://github.com/yuh-zha/AlignScore}}, which reports the performance of different metrics in evaluating factual consistency. %By offering this information, these leaderboards allow researchers and practitioners to make informed decisions about evaluation metrics. 
%     % \item \textbf{Method-oriented (or algorithm-oriented) leaderboards} focus on comparing ML algorithms (\ie, specific techniques or procedures used within the context of FMs) in a selective set of benchmarks under consistent model implementation. A representative example is the TOFU Leaderboard\footnote{\url{https://huggingface.co/spaces/locuslab/tofu_leaderboard}}, which reports the performance of model unlearning methods. % https://github.com/foundation-multimodal-models/CAL
%     \item \textbf{Solution-oriented (or service-oriented) leaderboards} allow stakeholders to identify specific entities, such as endpoint providers and competition participants, that deliver top-performing (in terms of effectiveness and/or popularity) solutions or services for a selective set of benchmarks. Representative examples are Papers Leaderboard\footnote{\url{https://huggingface.co/spaces/ameerazam08/Paper-LeaderBoard}\label{footnote:Papers Leaderboard}}, Provider Leaderboard\footnote{\url{https://leaderboard.withmartian.com}\label{footnote:Provider Leaderboard}} as well as those hosted on platforms such as Kaggle\footnote{\url{https://www.kaggle.com/competitions}}, EvalAI\footnote{\url{https://eval.ai}}, and Taostats\footnote{\url{https://taostats.io}}. The former reports the performance-cost tradeoff of different inference endpoint providers under resource-intensive conditions, while the latter offers competition-oriented leaderboards that encourage participants to develop innovative solutions for various benchmarks. %By offering this information, these leaderboards allow researchers and practitioners to identify the model providers that consistently deliver the best solutions. 
%     \item \textbf{Meta (or leaderboard-oriented) leaderboards} focus on comparing leaderboards based on their recognition or other attributes in the AI community. A representative example is the Open Leaderboards Leaderboard\footnote{\url{https://huggingface.co/spaces/mrfakename/open-leaderboards-leaderboard}}, a leaderboard of the top model-oriented leaderboards hosted in HF by popularity. %By offering this information, these leaderboards allow researchers and practitioners to identify the most suitable leaderboards for their specific needs and interests. 
% \end{itemize}

% It is essential to note that our classification of leaderboards is not mutually exclusive, as some platforms may combine characteristics of multiple types to achieve a more comprehensive goal. A prime example is SuperGLUE\footnote{\url{https://super.gluebenchmark.com/leaderboard}\label{footnote:SuperGLUE}}, which not only ranks model performance on various benchmarks (model-oriented), but also emphasizes the contributions made by each participating team (solution-oriented). 

% In this study, we focus on model-oriented leaderboards due to their widespread prevalence and importance for AI practitioners, specifically SE teams. These leaderboards play a vital role in helping them make informed decisions during the selection of appropriate FMs for various development tasks and their subsequent integration into final products. This is in line with the growing relevance of AI in SE (\ie, AI4SE~\cite{mcdermott2020ai4se}) and the growing need for effective tools, such as leaderboards, to help professionals in this interdisciplinary field.

% Besides the integration of evaluation records (what we mainly research in this study), benchmarks\footnote{\url{https://hub.opencompass.org.cn/dataset-submit}}, evaluators\footnote{\url{https://github.com/tatsu-lab/alpaca_eval?tab=readme-ov-file\#contributing-an-evaluator}}, and completion function\footnote{\url{https://github.com/tatsu-lab/alpaca_eval?tab=readme-ov-file\#contributing-a-completion-function}}, emphasize the recent efforts by leaderboard operators to address evaluation challenges—such as ``leaderboard plateauing''\footref{footnote:leaderboard plateauing} (also known as ``benchmark saturation''\cite{ott2022mapping,maslej2023artificial}) and ``inefficient benchmarking''\cite{polo2024tinybenchmarks}) by continuously adding, removing, and updating benchmarks through dedicated submission channels. Although these cases are currently limited, their increasing prevalence signifies a burgeoning trend that would enrich and complement our work. Investigating these evolutions (\ie, Progress Tracker\footnote{\url{https://huggingface.co/spaces/andrewrreed/closed-vs-open-arena-elo}\label{footnote:Progress Tracker}}) can lead to a more comprehensive understanding of LBOps, ultimately promoting more effective and dynamic leaderboard operations in the future.

% As of \collectdate, our approach has identified $1,045$ unique FM leaderboards, distributed across various combinations of hosting platforms illustrated in Figure~\ref{fig:platform}. In particular, PWC is the most popular platform, hosting up to $61.86\%$ ($446/1,045$) leaderboards. This is followed by HF ($16.64\%$), GitHub ($16.64\%$), and independent platforms ($13.31\%$). Furthermore, $7.91\%$ leaderboards are hosted on multiple platforms. It is worth mentioning that some cases involve multiple leaderboards hosted on the same website, such as the SuperCLUE series\footnote{\url{https://www.superclueai.com}\label{footnote:SuperCLUE}}, where each leaderboard has its own GitHub repository and is released on different dates for different tasks. 

% For RQ1, we examine the submission/contribution protocols, documentation/publication (\eg, blogs, reports), and commit history of these leaderboards. This helps us abstract common elements and identify key interactions and operational workflows. We chose submission/contribution protocols to understand how participants contribute to the leaderboards, while examining documentation/publication and commit history allows us to determine whether leaderboard operators are contributing to initial evaluation records. Initially, the first two authors randomly select $50$ leaderboards for analysis, of which they propose $7$ workflow patterns through the negotiated agreement technique~\cite{campbell2013coding}. Negotiated agreement involves iterative discussions and the building of consensus together among researchers. We also find that all PWC leaderboards adhere to a specific reference workflow, so we concentrate our in-depth analysis on non-PWC leaderboards in this RQ for a more comprehensive understanding of diverse LBOps.

% The first two authors then independently label workflow patterns of about $15\%$ ($40/278$) of the non-PWC leaderboards, achieving a Cohen's kappa inter-rater reliability score of $0.78$, indicating ``substantial agreement'' between the raters~\cite{gisev2013interrater}. Throughout the process, we maintain active communication with leaderboard operators through multiple channels, such as email, social networks (\eg, Slack\footnote{\url{https://slack.com}}, Discord\footnote{\url{https://discord.com}}, WeChat\footnote{\url{https://weixin.qq.com}}), and discussion forums, ensuring that any unclear documentation is clarified. Following additional conflict resolution among the authors, the first author designates the final labels on the remaining $85\%$ of non-PWC leaderboards. Whenever the first author identifies new workflow patterns, the first two authors negotiate new labels together. Through iterative discussion, we eventually consolidate $10$ highly similar workflows into $5$ unique workflow patterns that serve as the foundation of LBOps. Following this, we derive a domain model that effectively encapsulates the essential knowledge in LBOps using the unified modeling language~\cite{eriksson2000business} (UML) class diagram.

% Throughout the iterative backward snowball sampling phase (Phase~1) and the workflow pattern identification process, we uncover numerous recurring issues that emerge during leaderboard operations, spanning a wide range, from basic bugs that can be easily rectified to more critical fundamental flaws that require further scrutiny and resolution. To validate these issues, we report them to operators through discussion forums, emails, and WeChat. For example, we immediately raised an issue when we discovered that the submission panel was not responding to our requests on the KoLA leaderboard\footnote{\url{https://github.com/THU-KEG/KoLA/issues/17}}. As we receive more validation from the leaderboard operators on these issues, we introduce the concept of ``leaderboard smells'' to describe these phenomena that occur during LBOps to facilitate better understanding and management of the leaderboards.

% Throughout this process, we initiated $430$ GitHub issues, of which $301$ received responses from leaderboard operators, and $284$ were marked as resolved by us. Similarly, we created $332$ discussions on Hugging Face (HF), with $188$ receiving responses and $141$ being resolved. However, ambiguities sometimes persist in the feedback provided by the leaderboard operators. In such cases, we continued to make additional inquiries within the discussion threads, ensuring a thorough understanding of the issues at hand. This iterative process was repeated over several rounds until our concerns were fully addressed or no further responses were received from the operators. 

% For leaderboards that lack dedicated discussion forums, we joined their social networks, which included $4$ Discord channels, $3$ WeChat accounts, and $1$ Slack channel, enabling us to raise questions directly and facilitating $2$ phone calls to gain further clarity. For leaderboards without any of these communication channels, we established direct contact with operators by email, sending $14$ emails, and receiving responses from $8$ of them. These interactions allow us to validate our hypotheses regarding potential leaderboard smells and gather valuable insights from operators' feedback on maintaining their leaderboards.

% Having collected enough discussion posts, the first two authors periodically review each of them and collaboratively categorize leaderboard smells using the negotiated agreement technique~\cite{campbell2013coding}. In cases of ambiguity, we seek further clarification from leaderboard operators, ensuring that our confusion is effectively resolved. Due to the manual nature of detecting leaderboard smells, our study emphasizes identifying the presence of leaderboard smells rather than quantifying their severity or frequency across different leaderboard components. 

% Apart from identifying leaderboard smells, we actively collaborate with repository owners to address them by submitting pull requests to the relevant repositories. We submit a total of $12$ pull requests on GitHub, with $10$ merged. Additionally, we propose $7$ pull requests on HF, $4$ of which are merged. Collectively, these pull requests help resolve identified smells on up to $12$ leaderboards. For example, the ``fix medrxiv mislinkage'' pull request\footnote{\url{https://github.com/embeddings-benchmark/mteb/pull/187}} addresses an erroneous link redirection issue in MTEB. We limit our contributions to only a few pull requests due to the time-consuming nature of addressing complex smells. In addition, some smells originate from closed-source leaderboards, making them impossible to correct. Moreover, operators identify specific smells as ``not planned for now'', \ie, self-admitted technical debts, indicating that they lack the necessary resources or motivation to address these challenges (discussed in Section \ref{sec:rq2-results}). In general, our merge requests validate the practical relevance of our empirical findings, demonstrating their potential to improve the sustainability and trustworthiness of leaderboards in real-world scenarios. 

% We perform a multivocal literature review relevant to FM performance evaluation based on two sources to identify a comprehensive set of leaderboards.
% \begin{itemize}[leftmargin=*]
%     \item \textit{Google Scholar}\footref{footnote:Google Scholar}: We choose Google Scholar for its broad coverage of the academic literature, providing in-depth elaboration of the relatively novel concept of FM evaluation.
%     \item \textit{GitHub Awesome Lists}\footref{footnote:GitHub Awesome Lists}: We use GitHub Awesome Lists for their comprehensive collection of community-driven domain-specific resources, cataloging widely recognized benchmarks and leaderboards in the various domains. 
% \end{itemize}
%To prepare search queries on these two sources, we first compile a list of FM-related keywords through collaborative brainstorming between the authors and perform preliminary online searches, as presented in Table~\ref{tab:retrieved literature}. To optimize our search for relevant literature reviews on Google Scholar, we append our queries with various review-oriented terms, including ``review'', ``survey'', and ``study''. Additionally, for retrieving relevant GitHub Awesome Lists, we prefix each keyword with ``awesome'' to ensure that our search includes the awesome list repositories. 

% For Google Scholar, we only check the first $20$ pages of search results in each query to ensure a comprehensive, yet manageable analysis. For each piece of literature retrieved, we perform a preliminary skim to identify any sections dedicated to ML evaluation, ensuring that only relevant literature is selected for further analysis. Table~\ref{tab:retrieved literature} presents the collection of multivocal literature finalized from two sources through this systematic approach.

% \input{tables/method/retrieved-literature}

% To collect as many leaderboards as possible, we leverage the leaderboards and benchmarks in the collected multivocal literature. Then we employ an iterative backward snowball sampling algorithm~\cite{jalali2012systematic} to collect the leaderboards and associated benchmarks simultaneously. During this process, we only consider a platform as a leaderboard if the term ``leaderboard'' (or ``ranking/sorting table'') is explicitly mentioned in its documentation. For each identified leaderboard, we examine the corresponding documentation for references to other leaderboards or benchmarks, adding any new ones to our collection. Similarly, we search with Google for each benchmark to identify its provenance and any relevant leaderboards, which are then added to our leaderboard collection if they are new. This expansive process continues until all recognized leaderboards and their constituent benchmarks have been thoroughly explored, ensuring a comprehensive collection of leaderboards. Additionally, we expand our leaderboard collection by examining the PWC evaluation table dataset\footnote{\url{https://github.com/paperswithcode/paperswithcode-data}} and performing searches for the keyword ``leaderboard'' within HF Space\footnote{https://huggingface.co/spaces?sort=trending\&search=leaderboard}.

% In total, we identify six categories of ML leaderboards (detailed in Section~\ref{sec:background}), including $4$ dataset-, $1$ metric-, $1$ leaderboard-, $15$ method-, $1,062$ solution-, and $5,775$ model-oriented leaderboards. Our study focuses specifically on model-oriented leaderboards due to their dominating prevalence. In addition, model-oriented leaderboards are crucial resources for SE teams, enabling informed decision making when selecting the most suitable FMs for a wide range of tasks. We establish the following exclusion criteria for model-oriented leaderboards to enable a more focused analysis of LBOps for FMs.

% This comprehensive understanding serves as a solid foundation for addressing subsequent RQ. Finally, we present some leaderboard-related statistics to emphasize the prevalent characteristics relevant to leaderboard implementation. By recognizing and evaluating key operations in LBOps, we gain valuable insight into their strengths, weaknesses, and areas for improvement, thus establishing a solid foundation for the subsequent RQ. A domain model~\cite{fowler2012patterns} generally functions as an object model within a layer that utilizes a lower-level layer for persistence and provides an API to a higher-level layer, granting access to the model's data and behavior.  

% \item \emph{Leaderboards with one-time rankings}: These include evaluations found in various publication venues, such as blog posts, academic papers. This exclusion ensures that our analysis remains focused on leaderboards that are continuously evolving.
    % \item Leaderboards without numerical display. This exclusion guarantees that our analysis remains focused on quantitatively measurable results, ensuring rigor and precision in our evaluations. For example, we exclude the Meta Open LLM leaderboard\footnote{\url{https://huggingface.co/spaces/felixz/meta_open_llm_leaderboard}}.
    % \item Obsolete versions of leaderboards. For example, https://huggingface.co/spaces/malhajar/OpenLLMTurkishLeaderboard, https://huggingface.co/spaces/open-llm-leaderboard-old/open_llm_leaderboard. This exclusion ensures that our study reflects the state of practice in the field.
    % \item Leaderboards that are not designed for practical reference purposes. This exclusion ensures that our analysis remains focused on leaderboards for real-world applications and reference usage. For example, we exclude the ``Base Tests'' leaderboards in EvalPlus\footnote{\url{https://evalplus.github.io/leaderboard.html}\label{footnote:EvalPlus}}.
    % \item \emph{Leaderboards that restrict our collection process}: For example, the OPUS-MT leaderboard set its restriction to display only $50$ evaluations at maximum for any benchmark option\footnote{\url{https://github.com/Helsinki-NLP/OPUS-MT-dashboard/issues/2}}. This cap considerably narrows the scope of our analysis by precluding access to all evaluation records.
    % \item Non-model-oriented leaderboards. This exclusion guarantees that our analysis focuses on the operational aspects of model benchmarking and performance comparison. 
    
% While useful, existing leaderboards face challenges in standardizing and efficiently comparing the risks and limitations of top FMs~\cite{maslej2024artificialintelligenceindexreport}. Moreover, each leaderboard may follow distinct workflows with unique resource constraints and operational challenges, requiring additional efforts from operators to manage. For example, Open LLM Leaderboard operators have raised concerns about the time-intensive process of evaluating models, as assessing a $7B$ model on $8*H100 (80G)$ GPUs currently takes $2-3$ hours\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open_llm_leaderboard/discussions/801}}. Given the more than $7k$ FMs ranked in that leaderboard, its operators previously had to discontinue the DROP~\cite{dua2019drop} benchmark, as rerunning all evaluations was prohibitively expensive\footnote{\url{https://huggingface.co/blog/open-llm-leaderboard-drop}\label{footnote:DROP}}. In response to these challenges, the Open LLM Leaderboard has introduced a community-driven voting system, enabling maintainers to prioritize the order in which candidate models are evaluated\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/blog}\label{footnote:leaderboard plateauing}}. 


% \begin{table}[t]
% \centering
% \caption{Finalized multivocal literature on FM evaluation.}
% \label{tab:retrieved literature}
% \begin{NiceTabular}{l|C{2cm}|C{2cm}}
% \toprule
% \textbf{Primary Keyword} & \makecell{\textbf{GitHub} \\ \textbf{Awesome} \\ \textbf{Lists}} & \textbf{Google Scholar} \\
% \midrule
% benchmark & \cite{awesome-time-series-database,awesome-state-of-depth-completion,awesome-bioinformatics-benchmarks,Awesome_Satellite_Benchmark_Datasets,Awesome-LLM-Eval} & \\
% \midrule
% dataset & \cite{awesome-public-datasets,awesome-satellite-imagery-datasets,awesome-json-datasets,awesome-virtual-try-on,awesome-slam-datasets,awesome-diarization,Awesome-Cybersecurity-Datasets,awesome-instruction-dataset,Awesome-Knowledge-Graph-Reasoning,awesome-twitter-data,Awesome-Video-Datasets,awesome-reid-dataset,awesome-lidar,awesome-gee-community-datasets,awesome-biomechanics,Awesome-Deep-Graph-Clustering,awesome-chatgpt-dataset,game-datasets,awesome-chinese-legal-resources,Awesome-Deepfakes-Detection,awesome-segmentation-saliency-dataset,Awesome_Underwater_Datasets,Vehicle_reID-Collection,awesome-msr,awesome-industrial-machine-datasets,awesome-public-real-time-datasets,awesome-robotics-datasets,awesome-instruction-datasets,awesome-public-streaming-datasets,Awesome-Deep-Graph-Anomaly-Detection,Awesome-Traffic-Agent-Trajectory-Prediction,Awesome_Satellite_Benchmark_Datasets,awesome-colour,Awesome-instruction-tuning,awesome-bio-datasets,awesome-hungarian-nlp,Awesome-LLM-Eval,awesome-llm-human-preference-datasets,awesome-football,awesome-chemistry-datasets,Awesome_Multimodel_LLM,awesome-rgbd-datasets,Awesome-3D-LiDAR-Datasets,awesome-remote-sensing-change-detection} & \\
% \midrule
% leaderboard &&\\
% \midrule
% \multirow{2}{*}{foundation model} & \cite{Awesome-Remote-Sensing-Foundation-Models,Awesome-Reasoning-Foundation-Models,Awesome_Multimodel_LLM} & \cite{sun2023survey,zhou2023comprehensive,liu2023towards,rawte2023survey} \\
% \midrule
% \multirow{2}{*}{large action model}  & & \cite{wang2023survey,cui2024survey,zhao2023survey,xi2023rise} \\
% \midrule
% large AI model  & & \cite{qiu2023large} \\
% \midrule
% large audio model & \cite{awesome-large-audio-models} &  \\
% \midrule
% large audio language model &&  \\
% \midrule
% large behavior model &&  \\
% \midrule
% \multirow{10}{*}{large language model} & \cite{Awesome-LLM-Eval,Awesome-Multimodal-Large-Language-Models,LLM4Rec-Awesome-Papers,Awesome-LLM-for-RecSys,Awesome-LLM-3D,awesome-llm-and-aigc,Awesome-Story-Generation,Awesome-LLM4IE-Papers,Awesome_Multimodel_LLM,Awesome-LLMs-Evaluation-Papers,Awesome-Efficient-LLM} & \cite{wang2024exploring,chang2023survey,zhao2023survey,xi2023rise,qiao2022reasoning,wang2023survey,zhang2023instruction,shen2023large,cui2024survey,kalyan2023survey,zhu2023survey,zhang2023siren,zhao2023depth,guo2023evaluating,gallegos2023bias,wu2023multimodal,huang2023survey,yang2023survey,feng2023trends,wang2023knowledge,wei2022graph,dong2022survey,rawte2023survey,cao2024life,liu2023towards,fan2023trustworthiness,naveed2023comprehensive} \\
% \midrule
% large multimodal model & \cite{Awesome-Multimodal-Large-Language-Models,Awesome_Multimodel_LLM} & \cite{cui2024survey,wu2023multimodal} \\
% \midrule
% large speech model &&  \\
% \midrule
% large time series model &&  \\
% \midrule
% large trajectory model &&  \\
% \midrule
% large vision model & \cite{awesome-llm-and-aigc} & \cite{cui2024survey,lee2024foundation} \\
% \midrule
% small language model &&  \\
% \bottomrule
% \end{NiceTabular}
% \end{table}


% \item We contribute $311$ new dataset profiles in PWC\footnote{\url{https://paperswithcode.com/contribute/dataset/new}\label{footnote:pwc:dataset}}, improving the accessibility of critical benchmark dataset metadata for AI researchers.
    % \item We contribute to $12$ leaderboards by submitting $9$ pull requests ($8$ merges) on GitHub and $7$ pull requests ($4$ merges) on HF, demonstrating our commitment to fostering more robust and effective comparison of FMs practices in practical settings.
    % \item We describe a detailed categorization of leaderboards into model-, dataset-, leaderboard-, method-, metric-, and solution-oriented classes, each tailored for distinct evaluation purposes.

% Foundation models~\cite{bommasani2021opportunities} (FMs), also known as ``large AI models''~\cite{el2022impossible}, represent a paradigm-breaking change in the development of AI-driven software systems. Traditionally, machine learning (ML) models were trained on task-specific data, constraining their utility to a limited range of applications. FMs are large-scale ML models trained in extensive and diverse datasets, enabling them to adapt and fine-tune for various downstream tasks, such as code completion~\cite{dakhel2023github,barke2023grounded}, code understanding~\cite{nam2024using}, and software development~\cite{qian2023communicative}. The widespread adoption of techniques, such as fine-tuning~\cite{church2021emerging}, knowledge distillation~\cite{gou2021knowledge}, and reinforcement learning from human feedback~\cite{christiano2017deep} (RLHF), has led to the creation of hundreds of thousands of FM variants. This remarkable flexibility has presented a new challenge for FM users: identifying the most suitable FMs from the multitude of available options while considering crucial factors, such as deployment cost, inference latency, context window size, model capabilities, fine-tunability, commercial licensing, and other essential dimensions\footnote{This notation refers to a website, blog post, or issue report with its URL provided in the supplementary material of online replication package~\cite{replication_package}.}\footnote{\url{https://aws.amazon.com/blogs/machine-learning/fmops-llmops-operationalize-generative-ai-and-differences-with-mlops}\label{footnote:FMOps}}. 

% One potential solution to address this challenge is the use of FM leaderboards, such as the Big Code Models Leaderboard~\footref{footnote:Big Code Models Leaderboard}, which are centralized software systems designed to track and rank FMs based on the various factors mentioned above. These platforms aim to help data scientists, software developers, and other stakeholders efficiently select the most suitable FM candidates for testing and integration according to their specific application requirements. The concept of leaderboards\footnote{\url{https://huggingface.co/docs/leaderboards}} has progressed significantly from basic spreadsheets or static tables to intricate software systems hosted on cloud platforms, including Hugging Face (HF) Spaces\footnote{\url{https://huggingface.co/spaces}\label{footnote:Hugging Face Space}}, GitHub Pages\footnote{\url{https://pages.github.com}}, and Papers With Code (PWC)\footnote{\url{https://paperswithcode.com/sota}\label{footnote:pwc}}. These applications are built with complex operational workflows (\ie, processes to keep the leaderboards functional and reliable) that ensure continuous, objective, and valid evaluation data updates, transforming them into vital tools for systematic and reliable performance comparisons of participating models. Successful leaderboards come with their independent communities for vetting evaluations or submission artifacts, discussing leaderboard results, and publishing benchmarking insights in the academic literature.

% While useful, existing leaderboards face challenges in standardizing and efficiently comparing the risks and limitations of top FMs~\cite{maslej2024artificialintelligenceindexreport}. Moreover, each leaderboard may follow distinct workflows with unique resource constraints and operational challenges, requiring additional efforts from operators to manage. For example, Open LLM Leaderboard operators have raised concerns about the time-intensive process of evaluating models, as assessing a $7B$ model on $8*H100 (80G)$ GPUs currently takes $2-3$ hours\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open_llm_leaderboard/discussions/801}}. Given the more than $7k$ FMs ranked in that leaderboard, its operators previously had to discontinue the DROP~\cite{dua2019drop} benchmark, as rerunning all evaluations was prohibitively expensive\footnote{\url{https://huggingface.co/blog/open-llm-leaderboard-drop}\label{footnote:DROP}}. In response to these challenges, the Open LLM Leaderboard has introduced a community-driven voting system, enabling maintainers to prioritize the order in which candidate models are evaluated\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/blog}\label{footnote:leaderboard plateauing}}. 


% We use a three-stage methodology to achieve our study goal. First, we conduct a comprehensive multivocal literature review on the evaluation of FMs in GitHub~Awesome~Lists\footnote{\url{https://github.com/topics/awesome-list}\label{footnote:GitHub Awesome Lists}} and Google~Scholar\footnote{\url{https://scholar.google.com}\label{footnote:Google Scholar}}. Next, we extract benchmarks and leaderboards identified through the literature review and iteratively expand our data collection using backward snowball sampling~\cite{jalali2012systematic}. We also include leaderboards hosted on HF Space and PWC as supplementary sources. Lastly, we employ a multifaceted approach to analyze the collected leaderboards. This involves examining leaderboards, documentation, and publications, as well as engaging in direct communication with leaderboard operators when necessary. Throughout the process, we apply card sorting~\cite{wood2008card}, followed by negotiated agreement~\cite{campbell2013coding} between the authors to ensure a comprehensive data analysis.

% To our knowledge, this study is the first to examine the operationalization of ML leaderboards (\ie, ``leaderboard operations'') and to identify their common issues, referred to as ``leaderboard smells''. Our definition of ``Leaderboard Operations'' (LBOps) describes the resources and workflows needed to rank third-party ML models based on their evaluation performance and to help select the most suitable model candidates for a given context. LBOps complements MLOps~\cite{kreuzberger2023machine}, as the former focuses on the processes required to submit, evaluate, and compare \textbf{third-party} ML models, while the latter concentrates on training, versioning, and deploying \textbf{in-house} ML models. Together, LBOps and MLOps contribute to optimizing and managing ML workflows. In addition to defining LBOps, our paper contributes the following to the software engineering (SE) community based on a dataset of $1,045$ FM leaderboards:

% External contributors (\includegraphics[height=\baselineskip]{figures/rq1/EC.png}) submit their models (\includegraphics[height=\baselineskip]{figures/rq1/MS.png}) to a leaderboard through designated channels. In some cases, models (\includegraphics[height=\baselineskip]{figures/rq1/M.png}) are directly selected by the leaderboard operators (\includegraphics[height=\baselineskip]{figures/rq1/LO.png}). Following submission, the models undergo a pairwise output comparison process, where independent reviewers (\includegraphics[height=\baselineskip]{figures/rq1/IR.png}), either FMs (\eg, Auto-Arena\footnote{\url{https://huggingface.co/spaces/Auto-Arena/Leaderboard}\label{footnote:Auto-Arena}}) or human beings (\eg, Chatbot Arena\footnote{\url{https://lmarena.ai}\label{footnote:Chatbot Arena}}), serve as judges to evaluate the models. Reviewers perform inferences (\includegraphics[height=\baselineskip]{figures/rq1/MI.png}) on two models simultaneously by issuing designated or arbitrary requests. They conduct blind tests to compare the outputs, either between candidate models or against a baseline model. The output comparison occurs in two modes: ``peer battle'' and ``committee discussion''. In peer battle mode, reviewers directly evaluate the models~\cite{zheng2024judging}, while in committee mode, the process involves a series of comparative analyses and discussions among the reviewers~\cite{zhao2024auto}. In both modes, reviewers cast votes for the preferred model (\includegraphics[height=\baselineskip]{figures/rq1/OC.png}) based on the generated outputs (\includegraphics[height=\baselineskip]{figures/rq1/O.png}), choosing the model with the more satisfactory results or indicating a tie if neither is clearly superior. The aggregated reviewer preferences from multiple rounds are used to generate additional evaluation metrics (\includegraphics[height=\baselineskip]{figures/rq1/E.png}), such as Elo rating (\eg, Chatbot Arena~\cite{zheng2024judging}) and human alignment rate (\eg, Auto-J~\cite{li2023generative}). Finally, the evaluation records (\includegraphics[height=\baselineskip]{figures/rq1/E.png}) are integrated (\includegraphics[height=\baselineskip]{figures/rq1/CI.png}) into new or existing ranking dataframes (\includegraphics[height=\baselineskip]{figures/rq1/R.png}) for future releases (\includegraphics[height=\baselineskip]{figures/rq1/RI.png}). \\ 

% This pattern facilitates the continuous update of leaderboards with evaluation scores from diverse sources, contributing to a more comprehensive representation of model performance. However, the quality and reliability of extracted or submitted evaluations may vary due to a lack of structured reviewing of evaluation scores, potentially impacting the overall accuracy and trustworthiness of the leaderboard. For example, we find several common issues with the extracted evaluations in PWC leaderboards (as detailed in Section~\ref{sec:rq2-results}), which may result from inaccurate automated extraction\footnote{\url{https://github.com/paperswithcode/axcell}\label{footnote:axcell}} and PWC's ad hoc editing mechanism that permits any registered user to submit, remove, or modify values on the leaderboards.

%Due to the inherent complexity of natural languages, the mathematical evaluation of ML models is usually an ill-posed task~\cite{gudivada2015big}.

% The recognition of LBOps as its own discipline presents opportunities for researchers to improve the dynamics and sustainability of leaderboards. Researchers can work towards establishing standardized processes and best practices for the major workflows of leaderboards. This entails creating clear guidelines and protocols, such as ``leaderboard cards'' (analogous to repository cards\footnote{\url{https://huggingface.co/docs/huggingface_hub/package_reference/cards}}), that can be universally adopted to ensure consistent and reliable documentation of model ranking across different leaderboards. Additionally, researchers should develop specialized toolchains to automate model evaluation, ranking, and review processes, while also creating tools for detecting and addressing leaderboard smells. all *Ops disciplines foster collaboration between stakeholders that traditionally have been working in isolation, like developers and operators (DevOps) or data scientists and operators (MLOps) -> talk about the communities brought together by LBOps

% intelligent agents' internal representations of beliefs and understanding about tasks~\cite{el2015machine}

% This widespread distribution of smells critically undermines both the functionality and usability of leaderboards, necessitating immediate and targeted enhancements to ensure reliability and maintainability. 

% This is achieved by focusing exclusively on the evaluation of the prediction outputs. However, it is important to note that the data leakage~\cite{hannun2021measuring,shabtai2012data} problem still remains a potential threat to this workflow pattern, which may need to be addressed through appropriate measures. Each workflow pattern offers a unique balance of advantages and trade-offs, emphasizing specific aspects such as resource efficiency, data security, or transparency.

% Using this dual-ranking mechanism, SuperGLUE successfully functions as a model-oriented and solution-oriented leaderboard, highlighting the versatility and adaptability of these platforms in catering to the diverse requirements of FM reporting. The heterogeneity of the leaderboards mirrors the diverse practices and objectives found within the FM reporting landscape, showcasing the wide range of approaches employed by the machine learning community to achieve various goals and functionalities. 

%We also find that $0.37\%$ ($1$ out of $271$) of the non-PWC leaderboards do not align with any specific pattern due to inadequate or unclear documentation on their submission details. In an effort to address these ambiguities, we have submitted issue reports to the respective leaderboard repositories; however, no responses have been received as of \discussiontdate. This lack of clarity and communication may suggest that these leaderboards are less actively maintained, underscoring the need for improved documentation and responsiveness from leaderboard administrators.

% \emph{Constraints in Leaderboard Collection}: Despite our efforts to cover a wide range of leaderboards, it is important to recognize that some leaderboards may not have been included in our dataset. Thus, the possible exclusion of smell across specific components, such as those not appearing in Table~\ref{tab:leaderboad smell} or those left unchecked in that table, should not be interpreted as definitive proof of their non-existence. To address this limitation and ensure a representative sample of leaderboards, we combine multivocal literature from GitHub Awesome Lists and Google Scholar, using an iterative backward snowball sampling method. This approach involves a systematic and comprehensive examination of the multivocal literature and HF to collect leaderboards, thus increasing the likelihood of providing valuable insights and answers to the research questions posed in our study.

%Given the widespread occurrence of leaderboard smells in multiple components, it becomes crucial to examine the possible root causes of these issues. We find that PWC employs a unique ad hoc editing mechanism for their leaderboards, allowing any user to submit, remove, or change values in the leaderboards. Although the leaderboard administrators claim that all user-added results are curated and only verified results are published, we still notice a significant number of smells in the published leaderboards\footnote{\url{https://github.com/paperswithcode/paperswithcode-client/issues/25}}. Therefore, it might be beneficial to explore additional safeguarding mechanisms to mitigate or prevent possible smells arising from user-edited results. Implementing such measures could further enhance the trustworthiness and reliability of these leaderboards and contribute to more accurate and credible AI reporting.

%Initially, we collect the multivocal literature relevant to FM evaluation from different venues. Next, we perform a snowball backward sampling to collect a comprehensive list of leaderboards. Finally, we analyze each collected leaderboard by examining documentation, reports, and source code, communicating with leaderboard administrators through issue reports, and negotiating between authors in the open-coding process. This systematic approach ensures a comprehensive evaluation of leaderboards and encourages collaboration with system administrators through an empirically grounded basis.

    % \item Reference workflow: We examine and categorize the underlying workflows that define the operations of FM leaderboards, enabling a more structured understanding of their functionalities and components.
    % \item Domain model: We develop a comprehensive domain model to provide a clear representation of key elements and relationships within FM leaderboards, facilitating effective analysis and decision making.
    % \item Operational smell: We identify and investigate the various issues and challenges, referred to as ``smells'', that arise during the operations of the FM leaderboards. Addressing these smells is crucial to optimizing the performance and reliability of these systems.
    
%By examining these critical dimensions of leaderboards, we aim to provide actionable insights for their design, deployment, and improvement within the machine learning domain. By examining these aspects, we aim to provide useful insights to the publishers, developers, and maintainers of the leaderboard, collectively called ``leaderboard administrators'', as well as other stakeholders, to improve the overall maintainability and trustworthiness of these systems. In particular, we describe a new discipline called \textbf{leaderboard operations (LBOps)} that involves methodologies, practices, and toolchain for managing, operating, and evolving FM leaderboards, underscoring the importance of addressing complex processes in their design, configuration, and maintenance. This concept recognizes the complex and interconnected stages that comprise the development lifecycle of leaderboards, including model submission, inference, evaluation, leaderboard integration, and its deprecation. % To our knowledge, our study is the first to conduct a systematic exploration of the components, operations, and smell in leaderboards. Through this pioneering effort, we seek to lay the foundation for more sophisticated and impactful evaluation practices that can keep up with the rapidly changing demands of ML research and development.

 % We define LBOps as a conceptual framework designed to identify and organize the essential processes required to effectively translate model evaluations into accessible and user-friendly rankings. In a similar vein to DevOps (\eg, canary deployment) and MLOps (\eg, continuous training) that enable the seamless release of source code into software products and ML models into real-world applications, There is an existing literature that focus on practical implementation and maintenance of leaderboards and their associated components and you name it LBOps. LBOps focuses on the operationalization of leaderboards and their supporting components. By streamlining the processes involved in presenting and comparing the performance of various foundation models, LBOps aims to address the challenges associated with evaluating and ranking FMs. As an emerging conceptual framework, LBOps offers a unique opportunity to standardize responsible AI reporting, improve transparency in AI systems, and empower stakeholders to make well-informed decisions based on comprehensive information. Furthermore, LBOps contributes to the overall advancement of the AI ecosystem by supporting the continuous improvement and refinement of FMs and their applications.

% One valuable resource on which ML practitioners can rely when selecting models for testing is the leaderboards. An FM leaderboard serves as a visual medium that reports model rankings based on their performance, scores, or achievements in various contexts, including industry, business, and academic research\footnote{\url{https://dictionary.cambridge.org/dictionary/english/leaderboard}}. Those leaderboards enable ML practitioners and researchers to evaluate, compare, and track the progress of FMs on specific tasks, encouraging competition and the development of more effective approaches~\cite{ott2022mapping}. Despite their utility, there are no studies that explore the operationalization of leaderboards along with their supporting components, such as evaluation harness and benchmarks. The significant lack of standardization in responsible AI reporting poses challenges in comparing the risks and limitations of the top models~\cite{perrault2024artificial}. 

% This study investigates the current practices of leaderboard operations specifically designed for foundation models (FM), emphasizing their crucial role in AI reporting. Our goal is to improve the understanding and maintainability of leaderboards through a detailed examination of their characteristics, operations, and common issues. To achieve this objective, we employ a multifaceted approach that begins with retrieving multivocal literature reviews on FM evaluation from Google Scholar and GitHub Awesome Lists. Building upon this foundation, we identify relevant leaderboards by leveraging backward snowball sampling techniques starting from the retrieved literature, further supplemented by leaderboards hosted on the Hugging Face Hub. Lastly, we perform a thorough analysis of the documentation, publication, and commit history of the collected $443$ leaderboards, supplemented by direct and indirect communication with their administrators. Our findings introduce a novel conceptual framework, called ``leaderboard operations'' (LBOps), for leaderboard deployment in real-world production. e also introduce the concept of ``leaderboard smell'', which refers to operational issues that can affect the maintainability and trustworthiness of leaderboards. Our study underscores the need for more standardized benchmarking practices to support responsible AI reporting.

% which collectively include $2,987$ ranking dataframes (see Section~\ref{sec:rq1-results} for details) with up to $83,496$ evaluation records\footnote{For each leaderboard, we uniformly transform all evaluation records into tables for analysis purposes.}

% \emph{Submission channel} is the designated pathway through which users can submit their model-related information to leaderboards. For example, the submission channel is located under the ``Submit'' tab in the Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}. The model information contains essential information about the submitted model, which can include but is not limited to the model's name, publisher, release date, type (\eg, fine-tuned or base model), parameter count, publication name, and repository linkage. Then, the leaderboard administrators review their model-related information and verify their model based on the submission guideline. When the model does not fit the submission guideline, then the model would not be accepted for further evaluation. An example is the requirement for HF users to adhere to the metadata format in their model cards\footref{footnote:model index}. After the model passes the review, it would be evaluated against the designated benchmarks via the evaluation harness. 

% \emph{Evaluation harness} is a suite of software tools and frameworks designed to comprehensively evaluate ML models against a predefined set of benchmarks~\cite{bommasani2023holistic}. For example, FastChat\footnote{\url{https://github.com/lm-sys/FastChat}} is the evaluation harness of LMSYS Chatbot Arena Leaderboard\footref{footnote:LMSYS Chatbot Arena Leaderboard}. In this context, a typical benchmark consists of a problem formulation (task), data samples (raw dataset), descriptive labels (ground truth), evaluation configurations (protocol), and a set of quantitative measures (metrics)~\cite{denton2020bringing,dueben2022challenges,thiyagalingam2022scientific}. The model evaluation has two steps: model inference and prediction evaluation. Firstly, the evaluation harness access to the designated model and make inferences on this model with the test dataset following the benchmark protocol. Next, the evaluation harness compares the prediction output against the ground truth for getting the evaluation metric values. Combining the model-related information with the evaluation results, we have the evaluation records ready for further integration into the new or existing ranking dataframes. 


% is a visual aggregation of multiple evaluation records, organized according to a specified ranking and/or filtering criteria. For instance, in the LMSYS Chatbot Arena Leaderboard\footref{footnote:LMSYS Chatbot Arena Leaderboard}, the table found under the ``Overall'' category within the ``Arena'' tab exemplifies a ranking dataframe. The filtering criteria outlines the configurations by which evaluation records are aggregated within the ranking dataframe. In the example mentioned above, there are two options for users in the tab bar: ``Arena'' and ``Full Leaderboard''. While the former also holds up to $11$ categories, such as ``Overall'', ``Coding'', and ``Chinese''. Users can typically interact with the option tabs or custom-specified filter, such as inputting model keywords in the search box\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard}}. On the other hand, the ranking criteria establishes the rules for ranking evaluated models based on their evaluation results. Still the same example, the ranking dataframe on default uses ``Rank (UB)'' to rank the evaluated models, which is defined by ``one + the number of models that are statistically better than the target model''. In particular, model A is statistically better than model B when A's lower-bound score is greater than B's upper-bound score (in 95\% confidence interval). Typically, users can also rank the models based on a particular column within the ranking dataframe by interacting with the column names directly. 


% \emph{Submission channel} is the designated pathway through which users can submit their model-related information to leaderboards. For example, the submission channel is located under the ``Submit'' tab in the Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}. The model information contains essential information about the submitted model, which can include but is not limited to the model's name, publisher, release date, type (\eg, fine-tuned or base model), parameter count, publication name, and repository linkage. Then, the leaderboard administrators review their model-related information and verify their model based on the submission guideline. When the model does not fit the submission guideline, then the model would not be accepted for further evaluation. After the model passes the review, it would be evaluated against the designated benchmarks via the evaluation harness. %These details provide crucial context for understanding the model's characteristics and provenance. 

% \emph{Evaluation harness} is a suite of software tools and frameworks designed to comprehensively evaluate ML models against a predefined set of benchmarks~\cite{bommasani2023holistic}. For example, FastChat\footnote{\url{https://github.com/lm-sys/FastChat}} is the evaluation harness of LMSYS Chatbot Arena Leaderboard\footref{footnote:LMSYS Chatbot Arena Leaderboard}. In this context, a typical benchmark consists of a problem formulation (task), data samples (raw dataset), descriptive labels (ground truth), evaluation configurations (protocol), and a set of quantitative measures (metrics)~\cite{denton2020bringing,dueben2022challenges,thiyagalingam2022scientific}. The model evaluation has two steps: model inference and prediction evaluation. Firstly, the evaluation harness access to the designated model and make inferences on this model with the test dataset following the benchmark protocol. Next, the evaluation harness compares the prediction output against the ground truth for getting the evaluation metric values. Combining the model-related information with the evaluation results, we have the evaluation records ready for further integration into the new or existing ranking dataframes. The filtering criteria outlines the configurations by which evaluation records are aggregated within the ranking dataframe. In the example mentioned above, there is two options for users in the tab bar: ``Arena'' and ``Full Leaderboard''. While the former also holds up to $11$ categories, such as ``Overall'', ``Coding'', and ``Chinese''. Users can typically interact the filtering options using predefined, such as switching to other tabs or categories, or custom-specified criteria, such as inputting model keywords in the search box\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard}} (\textit{filter(UserInteraction): RankingDataframe}).

% the default ranking dataframe is in the ``Overall'' category under the ``Arena'' tab. 

% \emph{Ranking dataframe} is a visual aggregation of multiple evaluation records, organized according to a specified ranking and/or filtering criteria. For instance, in the LMSYS Chatbot Arena Leaderboard\footref{footnote:LMSYS Chatbot Arena Leaderboard}, the table found under the ``Overall'' category within the ``Arena'' tab exemplifies a ranking dataframe. 



% These criteria define the rules and constraints for filtering and ranking the records, enabling users to analyze and compare model performance effectively. 


%  In contrast to the filtering protocol, the ranking protocol establishes the guidelines for ranking evaluated models. This facilitates customized comparisons between models based on specific benchmark metrics or model attributes. Continuing with the example of the LMSYS Chatbot Arena Leaderboard, the default ranking of models is determined by the upper bound of the confidence interval of the Elo rating. Typically, users can rank the models based on a particular column within the Ranking Dataframe by simply clicking on the desired column name (\textit{rank(UserInteraction): RankingDataframe}).


% \emph{Evaluation record} is the fundamental building block of a leaderboard. It typically comprises model-related information and a set of evaluation results derived from the aforementioned evaluation process. For integration, the leaderboard administrators follow the predefined ranking criteria along with the filtering criteria, if any. The ranking criteria 

% \emph{Evaluation record (EvaluationRecord)} is the fundamental building block of a leaderboard. It comprises model information (ModelInfo) and a list of evaluation results (EvaluationResult). 

% \emph{Benchmark} is a standardized set of tasks, raw datasets, and evaluation metrics designed to evaluate and compare the performance of various ML models. It consists of an evaluation task (\textit{EvaluationTask}), an evaluation protocol (\textit{EvaluationProtocol}), a dataset (\textit{Dataset}), labels (\textit{GroundTruth}), and a set of predefined evaluation metrics (\textit{List<EvaluationMetric>})~\cite{denton2020bringing,dueben2022challenges,thiyagalingam2022scientific}. 

%In this context, a benchmark consists of a task to define the evaluation goal, a protocol, a dataset (\textit{Dataset}), labels (\textit{GroundTruth}), and a set of predefined evaluation metrics (\textit{List<EvaluationMetric>})~\cite{denton2020bringing,dueben2022challenges,thiyagalingam2022scientific}.

% \emph{Evaluation harness (EvaluationHarness)} is a suite of software tools and frameworks designed to comprehensively evaluate ML models against a predefined set of benchmarks (\textit{List<Benchmark>})~\cite{bommasani2023holistic}. For example, FastChat\footnote{\url{https://github.com/lm-sys/FastChat}} is the evaluation harness of LMSYS Chatbot Arena Leaderboard. Upon receiving an evaluatable artifact from the submission channel, the evaluation harness could evaluate it against a particular benchmark, generating new evaluation results (\textit{evaluate(EvaluatableArtifact, Benchmark): List<EvaluationResult>}). 

% These channels enable seamless integration of user-contributed models, prediction outputs, and evaluation records into the leaderboard for performance analysis and comparison. For example, the submission channel is located under the ``Submit'' tab in the Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}. Here, users can provide information about their model repository hosted on HF. In other cases, submission channels may be implicit, as seen in the LMSYS Chatbot Arena Leaderboard, where leaderboard administrators collect model information using their venues. In certain scenarios, submitted artifacts undergo a review process by the leaderboard administrators, who determine whether to accept or reject the submission (\textit{review(SubmittableArtifact):Bool}). An example is the requirement for HF users to adhere to the metadata format in their model cards\footref{footnote:model index}. This ensures proper extraction by PWC platform, allowing for the seamless integration of evaluation records into the ranking dataframe (\textit{integrate(EvaluationRecord,RankingDataframe)}).

% \emph{Submittable artifact (SubmittableArtifact)} refers to any entity that can be submitted to leaderboards through designated channels. This can be a model, prediction output\footnote{\url{https://super.gluebenchmark.com/submit}}, or evaluation record\footref{footnote:LLM-Leaderboard}. Models may be in the form of binary compression files\footnote{\url{https://jwolpxeehx.feishu.cn/wiki/C6VfwvbmOiuVrokpJAgcJXUcnLh}}, model repositories\footref{footnote:Open LLM Leaderboard}, or API inference points. Prediction outputs, on the other hand, constitute the results of evaluating a model using testing prompts from established benchmarks.

% \emph{Submission channel (SubmissionChannel)} is the designated pathway through which users can submit artifacts to leaderboards. These channels enable seamless integration of user-contributed models, prediction outputs, and evaluation records into the leaderboard for performance analysis and comparison. For example, the submission channel is located under the ``Submit'' tab in the Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}. Here, users can provide information about their model repository hosted on HF. In other cases, submission channels may be implicit, as seen in the LMSYS Chatbot Arena Leaderboard, where leaderboard administrators collect model information using their venues. In certain scenarios, submitted artifacts undergo a review process by the leaderboard administrators, who determine whether to accept or reject the submission (\textit{review(SubmittableArtifact):Bool}). An example is the requirement for HF users to adhere to the metadata format in their model cards\footref{footnote:model index}. This ensures proper extraction by PWC platform, allowing for the seamless integration of evaluation records into the ranking dataframe (\textit{integrate(EvaluationRecord,RankingDataframe)}).

% \emph{Evaluatable artifact (EvaluatableArtifact)} refers to any entity that can be evaluated against a set of established benchmarks using the evaluation harness, resulting in new evaluation results. An evaluatable artifact is a model or prediction output.

% \emph{Evaluation result (EvaluationResult)} is the quantitative representation of a model's performance on a specific benchmark. It comprises the numeric evaluation score along with the benchmark information (BenchmarkInfo). The numeric evaluation score serves as the primary indicator of a model's performance on the benchmark. This value is typically obtained by applying the specified evaluation metric to the model's output, thereby quantifying its success in addressing the task at hand. The benchmark information encompasses essential details about the benchmark, which might include the benchmark's name, the task it addresses, the protocol used for evaluation, the metric employed for scoring, and other relevant information about the benchmark's constituents. These attributes enable a comprehensive understanding of the context in which the model's performance is measured. 

% \emph{Evaluation record (EvaluationRecord)} is the fundamental building block of a leaderboard. It comprises model information (ModelInfo) and a list of evaluation results (EvaluationResult). The model information component contains essential information about the evaluated model, which can include but is not limited to the model's name, publisher, release date, type (\eg, fine-tuned or base model), parameter count, publication name, and repository linkage. These details provide crucial context for understanding the model's characteristics and provenance.

% \emph{Evaluation result (EvaluationResult)} is the quantitative representation of a model's performance on a specific benchmark. It comprises the numeric evaluation score along with the benchmark information (BenchmarkInfo). The numeric evaluation score serves as the primary indicator of a model's performance on the benchmark. This value is typically obtained by applying the specified evaluation metric to the model's output, thereby quantifying its success in addressing the task at hand. The benchmark information encompasses essential details about the benchmark, which might include the benchmark's name, the task it addresses, the protocol used for evaluation, the metric employed for scoring, and other relevant information about the benchmark's constituents. These attributes enable a comprehensive understanding of the context in which the model's performance is measured. 

% \emph{Ranking dataframe (RankingDataframe)} is a visual aggregation of multiple evaluation records (\textit{List<EvaluationRecord>}), organized according to a specified filtering (\textit{FilteringProtocol}) and ranking protocol (\textit{RankingProtocol}). These protocols define the criteria for filtering and ranking the records, enabling users to analyze and compare model performance effectively. For instance, in the LMSYS Chatbot Arena Leaderboard\footref{footnote:LMSYS Chatbot Arena Leaderboard}, the table found under the ``Overall'' category within the ``Arena'' tab exemplifies a ranking dataframe. The filtering protocol outlines the criteria by which evaluation records are classified within the ranking dataframe. In the example mentioned above, the default filter is the ``Overall'' category under the ``Arena'' tab. Users can typically modify the filtering options using predefined, such as switching to other tabs or categories, or custom-specified criteria, such as inputting model keywords in the search box\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard}} (\textit{filter(UserInteraction): RankingDataframe}). In contrast to the filtering protocol, the ranking protocol establishes the guidelines for ranking evaluated models. This facilitates customized comparisons between models based on specific benchmark metrics or model attributes. Continuing with the example of the LMSYS Chatbot Arena Leaderboard, the default ranking of models is determined by the upper bound of the confidence interval of the Elo rating. Typically, users can rank the models based on a particular column within the Ranking Dataframe by simply clicking on the desired column name (\textit{rank(UserInteraction): RankingDataframe}).

% \emph{Submittable artifact (SubmittableArtifact)} refers to any entity that can be submitted to leaderboards through designated channels. This can be a model, prediction output\footnote{\url{https://super.gluebenchmark.com/submit}}, or evaluation record\footref{footnote:LLM-Leaderboard}. Models may be in the form of binary compression files\footnote{\url{https://jwolpxeehx.feishu.cn/wiki/C6VfwvbmOiuVrokpJAgcJXUcnLh}}, model repositories\footref{footnote:Open LLM Leaderboard}, or API inference points. Prediction outputs, on the other hand, constitute the results of evaluating a model using testing prompts from established benchmarks.

% \emph{Submission channel (SubmissionChannel)} is the designated pathway through which users can submit artifacts to leaderboards. These channels enable seamless integration of user-contributed models, prediction outputs, and evaluation records into the leaderboard for performance analysis and comparison. For example, the submission channel is located under the ``Submit'' tab in the Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}. Here, users can provide information about their model repository hosted on HF. In other cases, submission channels may be implicit, as seen in the LMSYS Chatbot Arena Leaderboard, where leaderboard administrators collect model information using their venues. In certain scenarios, submitted artifacts undergo a review process by the leaderboard administrators, who determine whether to accept or reject the submission (\textit{review(SubmittableArtifact):Bool}). An example is the requirement for HF users to adhere to the metadata format in their model cards\footref{footnote:model index}. This ensures proper extraction by PWC platform, allowing for the seamless integration of evaluation records into the ranking dataframe (\textit{integrate(EvaluationRecord,RankingDataframe)}).

% \emph{Benchmark (Benchmark)} is a standardized set of tasks, datasets, and evaluation metrics designed to evaluate and compare the performance of various ML models. It consists of an evaluation task (\textit{EvaluationTask}), an evaluation protocol (\textit{EvaluationProtocol}), a dataset (\textit{Dataset}), labels (\textit{GroundTruth}), and a set of predefined evaluation metrics (\textit{List<EvaluationMetric>})~\cite{denton2020bringing,dueben2022challenges,thiyagalingam2022scientific}. A task is the problem formulation of the benchmark, which defines the specific goals to be achieved or challenges to be addressed by ML models. The protocol is a set of guidelines, rules, or procedures that govern how ML models should be evaluated on a benchmark. A dataset is a collection of structured or unstructured data samples that serves as the foundation for evaluating ML models. A label is a descriptive tag or identifier assigned to a specific data instance within the raw dataset, typically indicating the ground truth or the correct outcome for a given input. A metric is a quantitative measure to evaluate the performance of ML models in a specific benchmark.

% \emph{Evaluatable artifact (EvaluatableArtifact)} refers to any entity that can be evaluated against a set of established benchmarks using the evaluation harness, resulting in new evaluation results. An evaluatable artifact is a model or prediction output.

% \emph{Evaluation harness (EvaluationHarness)} is a suite of software tools and frameworks designed to comprehensively evaluate ML models against a predefined set of benchmarks (\textit{List<Benchmark>})~\cite{bommasani2023holistic}. For example, FastChat\footnote{\url{https://github.com/lm-sys/FastChat}} is the evaluation harness of LMSYS Chatbot Arena Leaderboard. Upon receiving an evaluatable artifact from the submission channel, the evaluation harness could evaluate it against a particular benchmark, generating new evaluation results (\textit{evaluate(EvaluatableArtifact, Benchmark): List<EvaluationResult>}). 

% integrating DyVal~\cite{zhu2023dyval} and prompt engineering benchmark~\cite{zhu2023promptbench2}, 

%There are more than $5$ evaluation records whose model names are listed as ``none'' on the A-OKVQA leaderboard\footnote{\url{https://leaderboard.allenai.org/a-okvqa/submissions/public}}, leading to transparency concerns.

%CLiB lacks a clearly defined evaluation protocol in its documentation\footnote{\url{https://github.com/jeinlee1991/chinese-llm-benchmark/issues/19}}\footnote{\url{https://github.com/jeinlee1991/chinese-llm-benchmark/issues/17}}, leading to potentially unreproducible evaluation results.

% Some leaderboards share a common underlying infrastructure, as observed by those hosted by AI2\footnote{\url{https://leaderboard.allenai.org}\label{footnote:AI2}}, CRFM\footnote{\url{https://crfm.stanford.edu}}, PWC, and others. For example, the Demo leaderboard\footnote{\url{https://huggingface.co/spaces/demo-leaderboard/leaderboard}} provides boilerplate code that allows new users to generate and contribute to various leaderboards more easily. These include the Enterprise Scenarios leaderboard\footnote{\url{https://huggingface.co/spaces/PatronusAI/enterprise_scenarios_leaderboard}\label{footnote:Enterprise Scenarios leaderboard}}, the LLM Safety Leaderboard\footnote{\url{https://huggingface.co/spaces/AI-Secure/llm-trustworthy-leaderboard}\label{footnote:LLM Safety Leaderboard}}, and the Toxicity Leaderboard\footnote{\url{https://huggingface.co/spaces/Bias-Leaderboard/leaderboard}\label{footnote:Toxicity Leaderboard}}. The collaborative environment and code-sharing practices among these leaderboards foster a more streamlined development process, ultimately promoting efficiency and improving evaluation capabilities within the ML community.

% \emph{Evaluation record}: We find that the mean number of unique evaluation records in various leaderboards is $189.3$, with a median of $23$ and an IQR of $48$, underscoring a skewed distribution where a few leaderboards contain a large number of records while most have fewer. In particular, HELM (Classic)\footref{footnote:HELM (Classic)} has the highest number of unique evaluation records up to $16,005$, followed by LMExamQA\ref{footnote:LMExamQA} ($7,096$) and Open LLM Leaderboard (GPT)\footref{footnote:Open LLM Leaderboard (GPT)} ($5,839$). Moreover, $1.14\%$ ($5$ out of $441$) leaderboards contain empty leaderboards (\ie, without evaluation records).

% \emph{Leaderboard - Rank}: According to our leaderboard collection criteria (Section~\ref{sec:method:design}), each leaderboard is associated with at least one leaderboard. Our analysis reveals a mean of $6.8$ leaderboards per system, with a median of $1$ and an interquartile range (IQR) of $2$. These metrics highlight a skewed distribution, implying that while a few leaderboards may contain numerous leaderboards, the majority have relatively few. In particular, we find that LMExamQA\footref{footnote:LMExamQA} has the highest number of $887$ leaderboards. This is closely followed by HELM (Classic)\footref{footnote:HELM (Classic)} ($301$) and BIG-Bench\footnote{\url{https://paperswithcode.com/dataset/big-bench}\label{footnote:BIG-Bench}} ($127$).

% \emph{Leaderboard - display format}: We find that \textit{rankable table} proves to be the most prevalent display format for leaderboards, accounting for $77.45\%$ ($340$ out of $441$) leaderboards. This is closely followed by \textit{scatter plot} ($50.57\%$) and \textit{regular table} ($25.97\%$). Other formats, including \textit{bar chart} ($6.61\%$), \textit{table screenshot} ($4.78\%$), \textit{radar chart} ($1.14\%$), \textit{sortable bar chart} ($0.46\%$), \textit{line chart} ($0.46\%$), and \textit{heat map}, \textit{box plot}, and \textit{JSONL} both at $0.23\%$, are less frequently used. 

%The Enterprise Scenarios Leaderboard\footnote{\url{https://huggingface.co/spaces/PatronusAI/enterprise_scenarios_leaderboard/discussions/10}} and YALL\footnote{\url{https://huggingface.co/spaces/mlabonne/Yet_Another_LLM_Leaderboard/discussions/4}} introduce benchmarks that lack sufficient specifications and references, creating a critical context gap for users to understand the scope, methodology, and relevance of the benchmarks.

%\emph{Leaderboard - participating model}: After checking the model names within evaluation records, we find that the mean number of participating models in various leaderboards is $73.87$, with a median of $17$ and an IQR of $26$. These metrics imply a skewed distribution, indicating that a few leaderboards feature a large quantity of participating models, while the majority contain fewer. In particular, Open LLM Leaderboard (GPT)\footnote{\url{https://huggingface.co/spaces/gsaivinay/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard (GPT)}} has the highest number of participating models up to $5,485$. This is followed by the Open LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard}} ($5,291$) and the Open MLLM Leaderboard\footnote{\url{https://huggingface.co/spaces/Wwwduojin/MLLM_leaderboard}\label{footnote:Open MLLM Leaderboard}} ($4,634$). 

%\emph{Pull request channel}: We find that $54.21\%$ ($238$ out of $441$) leaderboards provide at least one pull request channel. In particular, PWC leaderboards do not support any pull request mechanism, highlighting a substantial difference in development practices compared to other platforms.

%\emph{Submission channel}: We find that $74.26\%$ ($326$ out of $441$) leaderboards provide at least one submission channel, including email\footnote{\url{https://eqbench.com}\label{footnote:EQ-Bench}}, evaluation harness\footnote{\url{https://huggingface.co/spaces/Cognitive-Lab/indic_llm_leaderboard}\label{footnote:Indic LLM Leaderboard}}, issue report\footnote{\url{https://github.com/ray-project/llmperf-leaderboard}\label{footnote:LLMPerf}}, model card\footnote{\url{https://mteb.info}\label{footnote:MTEB}}, pull request\footnote{\url{https://github.com/hendrycks/test}\label{footnote:MMLU}}, questionaire\footnote{\url{https://trustllmbenchmark.github.io/TrustLLM-Website/leaderboard.html}\label{footnote:TrustLLM}}, upload portal\footnote{\url{https://huggingface.co/spaces/gaia-benchmark/leaderboard}\label{footnote:GAIA}}, and WeChat\footnote{\url{https://www.superclueai.com}\label{footnote:SuperCLUE}}.

%\emph{Contact information}: We find that $99.77\%$ ($438$ out of $441$) leaderboards provide at least one type of contact information, with the only exception of OpenEval\footnote{\url{http://openeval.org.cn/\#/rank}\label{footnote:OpenEval}}.

%\emph{Discussion forum} We find that $54.21\%$ ($238$ out of $441$) leaderboards offer at least one discussion forum hosted on either GitHub or HF. In particular, PWC leaderboards are not associated with any discussion forums, highlighting a substantial difference in development practices compared to other platforms.

%\emph{Documentation}: We find show that $99.32\%$ ($436$ out of $441$) of the leaderboards are accompanied with documentation. 

%\emph{Benchmark}: We find that every leaderboard incorporates at least one benchmark for evaluation purposes.

%\emph{Evaluation harness}: We find that $56.26\%$ ($247$ out of $441$) leaderboards are associated with at least one evaluation harness. In particular, PWC leaderboards are not associated with any evaluation harnesses, suggesting a notable distinction in practices between these platforms. %; however, the public accessibility of these harnesses varies considerably

 

% \emph{Leaderboard} serves as a user interface, displaying the model rankings and relevant information (described below) in an organized and accessible manner. Leaderboards can be presented in various formats, including tables (\eg, table\footnote{\url{https://tatsu-lab.github.io/alpaca_eval}\label{footnote:AlpacaEval}}, rankable table\footnote{\url{https://huggingface.co/spaces/gsaivinay/open_llm_leaderboard}}, table screenshot\footnote{\url{https://github.com/MikeGu721/XiezhiBenchmark}\label{footnote:Xiezhi}}) or figures (\eg, bar chart\footnote{\url{https://leaderboard.tabbyml.com}\label{footnote:Coding LLMs Leaderboard}}, box plot\footnote{\url{https://artificialanalysis.ai/leaderboards/models}\label{footnote:Models Leaderboard}}, heat map\footnote{\url{https://github.com/Libr-AI/do-not-answer}\label{footnote:Do-Not-Answer}}, line chart\footnote{\url{https://xwang.dev/mint-bench}\label{footnote:MINT}}, pie chart\footnote{\url{https://osu-nlp-group.github.io/TravelPlanner}\label{footnote:TravelPlanner}}, radar chart\footnote{\url{https://huggingface.co/spaces/BramVanroy/open_dutch_llm_leaderboard}\label{footnote:Open Dutch LLM Evaluation Leaderboard}}, scatter plot\footnote{\url{https://huggingface.co/spaces/ml-energy/leaderboard}\label{footnote:ML.ENERGY Leaderboard}}, sortable bar chart\footnote{\url{https://huggingface.co/spaces/ramiroluo/LLMHallucination_Leaderboard}\label{footnote:LLMHallucination Leaderboard}}). Each format offers unique benefits for data visualization, enabling easy comparison or emphasizing critical performance metrics. Additionally, Leaderboards are stored in a range of file formats, including CSV (comma-separated values)\footnote{\url{https://allenai.org/project/a-okvqa/home}\label{footnote:A-OKVQA}}, JSON (JavaScript object notation)\footnote{\url{http://103.238.162.37:31622/LeaderBoard}\label{footnote:KoLA}}, XLSX (Microsoft Excel spreadsheet)\footnote{\url{https://huggingface.co/spaces/daishen/SCULAiW}\label{footnote:LAiW}}, TSV (tab-separated values)\footnote{\url{https://huggingface.co/spaces/mlfoundations/VisIT-Bench-Leaderboard}\label{footnote:VisIT-Bench}}, LATEX (Lamport's TeX)\footref{footnote:Open Dutch LLM Evaluation Leaderboard}, MD (markdown file)\footnote{\url{https://huggingface.co/spaces/allenai/reward-bench}\label{footnote:RewardBench}}, XLS (Excel spreadsheet)\footnote{\url{https://lmexam.com}\label{footnote:LMExamQA}}, and JSONL (JSON lines format)\footnote{\url{https://huggingface.co/spaces/allenai/URIAL-Bench}\label{footnote:URIAL-Bench}}, to suit different user preferences and requirements\footnote{We are only interested in the storage formats that are directly downloadable for users.}.

% Each leaderboard comprises an indefinite number of evaluation records generated through designated benchmarks. Each \textit{evaluation record} consists of the model name, context information, and evaluation results. The \textit{model name} functions as a unique identifier, comprising the official designation, version number, or distinct attributes for precise model identification. \textit{Context information} provides crucial background details that include model- or evaluation-specific contexts to facilitate a comprehensive understanding of the comparisons. The \textit{model context} includes details such as the model's publisher, release date, type (\eg, fine-tuned or base model), parameter count, related publications, and codebase. This spectrum of attributes enriches comprehension of the design, capabilities, and intended applications of participating models. The \textit{evaluation context} encompasses the details of the evaluation methodology, including the submission date, the evaluation strategy, and task-specific information. This offers insight into the evaluation's procedural nuances, enhancing the interpretation of evaluation results. The \textit{evaluation result} quantifies the model's performance based on the evaluation process, typically through metrics such as accuracy, precision, and recall. 

% \emph{Contribution avenues} include various channels that allow ML practitioners to contribute to developing leaderboards. These avenues include pull request and submission channels. \textit{Pull request channels} serve as a venue where developers can contribute to the leaderboard's development by proposing novel features, bug fixes, or improvements. \textit{Submission channels} provide a straightforward method for ML practitioners to contribute their models (\eg, Open LLM Leaderboard\footref{footnote:Open LLM Leaderboard}), predictions (\eg, GAIA\footnote{\url{https://huggingface.co/spaces/gaia-benchmark/leaderboard}}), evaluations (\eg LLM-Leaderboard\ref{footnote:LLM-Leaderboard}), or even benchmarks (\eg, OpenCompass Large Language Model Leaderboard\footnote{\url{https://hub.opencompass.org.cn/dataset-submit}}) directly to the leaderboard.

% \emph{Communication avenues} include various channels that facilitate the exchange of information between leaderboard administrators and users regarding leaderboards. Communication channels include contact information, discussion forums, documentation, and publication. \textit{Contact information} provides a direct means for practitioners to reach out to administrators for inquiries or feedback. This can include email addresses, social networks, or other contact details. \textit{Discussion forums} provide a space for practitioners and administrators to exchange ideas, insights, and feedback on leaderboards. \textit{Documentation} serves as a comprehensive resource for users to understand the architecture, components, and functionalities of the leaderboard. \textit{Publication}, including research papers, blog posts, and articles, provides in-depth insight into the design, goals, and implications of leaderboards, allowing practitioners to gain a deeper understanding of the system's context. 

% \emph{Evaluation Suite} is a curated collection of benchmarks and evaluation harnesses that provide a comprehensive set of tools for the standardized evaluation and comparison of models or methods within a specific domain. A \textit{benchmark} is a standardized testing framework used to evaluate and compare the performance of different ML models, algorithms, or systems~\cite{thiyagalingam2022scientific}. It consists of four key components: configuration, datasets, metrics, and tasks, which collectively establish a uniform testing environment to ensure fair and accurate performance evaluations~\cite{denton2020bringing,dueben2022challenges}. A \textit{task} is the problem formulation of the benchmark, which defines the specific goals to be achieved or challenges to be addressed by ML models. The \textit{configuration} is a set of guidelines, protocols, or procedures that govern how ML models should be trained, tested, and evaluated on a benchmark. A \textit{dataset} is a collection of structured or unstructured data samples, often labeled or annotated, that serves as the foundation for training, testing, and evaluating ML models. A \textit{metric} is a quantitative measure used to evaluate the performance of ML models in a specific benchmark. The \textit{evaluation harness} is a comprehensive suite of software tools and frameworks designed to evaluate ML models against benchmarks. 


% dataset: We find that $0.68\%$ ($3$ out of $441$) leaderboards do not provide predefined datasets for evaluation. In these exceptional cases, the evaluation relies on human judges who generate custom test prompts based on their individual preferences, highlighting the adaptability and flexibility of certain leaderboards. 

% \subsection{Types of Leaderboard Operation}

%Ultimately, this model serves as a valuable tool for advancing the effectiveness and efficiency of ML leaderboards to evaluate and compare model performance.

% \begin{itemize}[leftmargin=*]
%     \item \textit{Leaderboard Requirement} is the foundational stage in the leaderboard development workflow. This stage is crucial to define the purpose, goals, and essential features of the leaderboards. It involves a thorough assessment of the context in which the leaderboard would operate, the specific audience it aims to serve, and the critical performance metrics it is expected to measure. Throughout this phase, publishers collaborate to compile requirements, perform analysis of competing or similar solutions, and pinpoint any constraints that could influence the design and functionality of the leaderboard. The culmination of this stage is a detailed set of requirements and specifications that would guide the design, deployment, and ongoing maintenance of the leaderboards. Occasionally, this phase occurs informally without the production of formal documentation.
%     \item \textit{Leaderboard design} builds on the requirements established in the previous stage, focusing on creating the architecture and detailed design of the leaderboard. This involves selecting the appropriate data structures, algorithms, and technologies to efficiently store, process, and present the leaderboard information. The outcome of this stage is a detailed design specification that serves as a blueprint for the leaderboard implementation, guiding developers to build a robust and user-friendly system. The design phase typically requires collaboration between stakeholders, such as designers, developers, and data scientists, to ensure a comprehensive and well-thought-out solution. Sometimes, this phase occurs informally without the production of formal specification.
%     \item \textit{Leaderboard deployment} marks the stage when the designed leaderboard is implemented and launched in a production environment. This involves the process of building, coding, and setting up the leaderboard according to the predetermined design and specifications. During this phase, extensive testing is conducted to ensure that the leaderboards operate as intended and meets performance expectations. Once the deployment is complete, the leaderboards become accessible to its target audience, enabling users to view, analyze, and compare performance metrics. Occasionally, deployment occurs incrementally, with new features rolled out in stages, allowing for user feedback and iterative improvements. Different platforms offer varying levels of support to present leaderboards, each boasting unique features and capabilities. For example, GitHub provides two primary methods for leaderboard presentation: embedding tables or graphs directly into markdown files, such as ``README.md'' or utilizing GitHub Pages\footnote{\url{https://pages.github.com}} to create a dedicated website with a ``github.io'' URL suffix, facilitating a more customized and visually appealing presentation of leaderboards. In contrast, HF offers Spaces, a feature that allows users to build and showcase interactive leaderboards using infrastructure including Gradio\footnote{\url{https://www.gradio.app}}, Streamlit\footnote{\url{https://streamlit.io}}, and Docker Spaces\footnote{\url{https://huggingface.co/docs/hub/spaces-sdks-docker}}. HF Spaces enable seamless integration of data visualizations, performance metrics, and user engagement features, fostering a dynamic and immersive leaderboard experience. Additionally, PWC supplies a leaderboard template that demands essential model-specific details, including ``Model'' (model name), ``Paper'' (publication), ``Code'' (GitHub repository), ``Result'' (precise location of results within publication tables), ``Year'' (publication year), and ``Tags'' (model architecture or other classification). his comprehensive approach ensures that leaderboards remain informative, transparent, and easily navigable, ultimately enhancing user experience and facilitating data-driven decision-making.
%     \item \textit{Leaderboard maintenance} includes the ongoing management and support of the leaderboard post-deployment, such as bug fixes, feature requests, and continuous monitoring. Additionally, leaderboard maintenance includes incorporating new submissions, updating rankings, and managing user feedback or queries. To maintain optimal performance and meet evolving user needs, periodic updates to the system infrastructure, visual design, or benchmarks may be necessary. Our study focuses primarily on evaluation-related operations within the leaderboard maintenance phase. Regular communication with the user community is essential during this stage to keep the leaderboard relevant and valuable for its intended audience. The maintenance phase is typically an iterative process, requiring continuous attention and adaptation to ensure leaderboard functionalities.
%     \item \textit{Leaderboard deprecation} signifies the final stage in the leaderboard development workflow, where the leaderboard is retired or phased out. This stage may be necessitated by various factors, such as the emergence of more advanced evaluation techniques, changes in user preferences or requirements, or the discontinuation of the underlying technology. During the deprecation phase, the leaderboard administrators would typically notify users, archive the leaderboard's historical data and performance records, and potentially migrate users to alternative evaluation systems. 
%     \item \textit{Model selection} is a critical step in the leaderboard development workflow, involving the careful selection and collection of suitable ML models for evaluation. This stage entails a comprehensive assessment of the available models, considering factors such as model performance, complexity, alignment with leaderboard objectives, and novelty. By thoughtfully evaluating these aspects, leaderboard administrators can curate a diverse and representative collection of ML models that showcase the state-of-the-art in the field while promoting continuous progress and discovery within the ML community.
%     \item \textit{Model evaluation} is a critical step within the leaderboard development workflow, where the performance of ML models is evaluated against established benchmarks. Model evaluation can be broadly classified into two primary types, depending on the roles and benchmarks involved: automated and human-based evaluation. Automated evaluation employs ML models to generate predictions or decisions on previously unseen data, leveraging types learned during training. Subsequently, these predictions are compared against ground truth in supervised learning scenarios or judged against specific grading criteria, such as predefined metrics (\eg, perplexity~\cite{jelinek1977perplexity}) or FM-as-a-judge~\cite{zheng2024judging,chen2024mllm}. In comparison, human-based evaluation incorporates human preference in grading or comparing ML models, which can be further divided into two approaches: scoring models based on human preference\footnote{\url{https://github.com/jeinlee1991/chinese-llm-benchmark}\label{footnote:CLiB}} and conducting pairwise model comparisons~\cite{zheng2024judging}. The former approach evaluates models by attributing scores that mirror human judgment and inclination, while the latter employs pairwise comparisons to facilitate direct evaluation of model performance by human evaluators under blind test conditions. Both automated and human-based evaluation play significant roles in the leaderboard, enabling a comprehensive assessment of ML models to ensure their reliability, accuracy, and alignment with user expectations.
%     \item \textit{Submission review} is a critical step in the leaderboard developement workflow, ensuring that all submitted models, predictions, evaluations, and associated configuration files adhere to the established standards and guidelines set forth by the leaderboard administrators. However, it is essential to note that not all leaderboards have a formal submission review process in place. During this stage, leaderboard administrators meticulously evaluate the submitted artifacts, scrutinizing various aspects such as model architecture, prediction quality, evaluation metrics, and configuration files. The review process maintains the credibility and trustworthiness of the leaderboard by fostering a competitive yet collaborative environment that encourages participants to refine their models and contribute to the advancement of the ML field.
% \end{itemize}

% \subsection{Types of reference workflow}

% Our analysis of the collected leaderboards has revealed up to $10$ distinct types of reference workflow that align with the reference workflow. 

% Our findings would inform strategies for leaderboard administrators to improve operational efficiency and system robustness in LBOps.

% Finally, we refine the reference workflow to create an adaptable and abstract representation that accommodates all recognized patterns. For RQ2, inspired by Hassan~et~al.~\cite{hassan2000reference} and Grosskurth~et~al~\cite{grosskurth2005reference}, we propose a reference architecture for leaderboards based on the documentation and publications of collected systems. Additionally, we explore the component distribution within our collected leaderboards, providing empirical evidence to validate the proposed reference architecture. 

% emphasize the importance of understanding the broader context and interplay of these elements. In doing so, we strive to contribute to the standardization and enhancement of responsible AI evaluations in real-world scenarios.

%     +filter(EvaluationModel,EvaluationMetric)

% RankableDataframe "1" -- "0..*" EvaluationRecord
% Submission could be either an internal (Type1~5) or external submission (Type1,6~8). Rat


% EvaluationRecord "1" -- "1" ModelInfo
% EvaluationRecord "1" -- "*" EvaluationResult


% SubmissionChannel -- EvaluationHarness : passes >
% EvaluationHarness -- ReviewedArtifact : receives >
% RankingDataframe -- EvaluationRecord : ranks >

% , identifying the most effective algorithmic approaches 

% Leaderboards serve as indispensable resources for ML stakeholders when selecting appropriate models for testing. These visual interfaces rank models based on performance, scores, or achievements in diverse contexts, including industry, business, and academic research\footnote{\url{https://dictionary.cambridge.org/dictionary/english/leaderboard}}. ML leaderboards enable developers and researchers to assess, compare, and monitor the progress of ML models on specific tasks, promoting competition and driving the development of more advanced algorithms~\cite{ott2022mapping}. By isolating the effectiveness of models as the primary variable, these leaderboards maintain consistency in other factors, such as datasets, metrics, and prompt engineering, allowing for a fair evaluation of model performance. 

%In particular, certain primary keywords are excluded from the table due to the absence of multivocal literature on FM evaluation. Our in-depth analysis of the collected literature reveals a strong interconnection between benchmarks and leaderboards. This insight leads us to develop a systematic approach in Phase~2, focusing on the exploration and exploitation of leaderboards and their associated benchmarks.

% With a basic understanding of the leaderboards, we now explore the existing literature on evaluations in computer science. Weber~et~al.~\cite{weber2019essential} provide essential guidelines for designing, performing, and interpreting benchmarking studies in computer science, with a focus on computational biology. The guidelines cover various aspects such as defining the purpose and scope of the benchmark, including all relevant methods, selecting representative datasets, choosing appropriate parameter values and software versions, evaluating methods using key performance metrics, considering secondary measures such as computational requirements and user-friendliness, interpreting results from both user and method developer perspectives, releasing results in an accessible format, designing benchmarks for future extensions, and following reproducible research best practices. In contrast, our research investigates the structural components, operational dynamics, and challenges encountered in leaderboard systems. Our findings provide distinctive insights and recommendations to improve the development of leaderboards in this specific context, providing a targeted complement to the broad principles outlined in the study mentioned above.

% Höllig~et~al.~\cite{hollig2020individualizing} investigates the relationship between the competitiveness of user traits and their participation in gamified systems, focusing on how different leaderboard designs (team-based versus player-based) influence user interaction. They explore both direct and indirect effects of personal development competitiveness on users' intention to use such systems, mediated by perceived enjoyment. The findings indicate an indirect relationship between trait competitiveness and usage intention through perceived enjoyment, which is further moderated by the system's leaderboard design. This research highlights the importance of aligning the design of the gamified system with user traits to improve user engagement. In contrast, we focus on exploring the structural components, operational dynamics, and challenges encountered in leaderboard systems to enhance transparency, fairness, and reproducibility in model evaluation. 

% Na~et~al.~\cite{na2023leaderboard} investigate how leaderboard positions affect motivation in gamified tasks. Through an online experiment in a crowd-sourcing context, they explore the behavioral and self-reported impacts of high versus low leaderboard positions on motivation, focusing on competence satisfaction and frustration. Their research reveals that elevated rankings can lead to complacency, while lower rankings tend to boost motivation, particularly in the absence of intrinsic motivation. Using the ``needs-as-motive'' model from self-determination theory~\cite{sheldon2009psychological}, their research contributes to a deeper understanding of the motivational dynamics at play in gamification contexts. In contrast, our paper makes a significant contribution by systematically exploring the operational dynamics of leaderboard systems, focusing on the variation of core practices across different evaluation workflows. Our study complements these broader principles by focusing on common problems (\ie, ``smell'') in leaderboard systems. 

% This review aims to identify key trends, methodologies, and findings in the field, highlighting their relevance and implications for our study. Ethayarajh~et~al.~\cite{ethayarajh2020utility} critique the traditional focus on performance-based evaluation in natural language processing (NLP) leaderboards, highlighting the limitations of only prioritizing accuracy metrics. The authors argue that this approach neglects other important qualities valued by the NLP community, such as fairness, energy efficiency, and robustness. They propose a framework of utility theory to better align leaderboards with the preferences of practitioners, emphasizing the need for transparency and reporting of relevant statistics, such as model size and inference latency. By reframing the discussion around utility and advocating for a more holistic evaluation approach, the article aims to bridge the gap between leaderboard incentives and the practical needs of NLP practitioners. In cosntract, our goal is to dissect leaderboard systems by looking at how evaluation records are organized, understanding the distribution patterns of components, and identifying prevalent smell. 

% Until now, most studies in software engineering (SE) related to FM have focused on using FMs to enhance SE tasks~\cite{feng2024prompting,xia2023automated,fan2023automated}, or employing SE techniques to improve the FM development process~\cite{arawjo2023chainforge,pang2024ai2apps,shankar2024spade}. These studies typically originate from disciplines outside the traditional SE community, focusing more on theoretical or methodological advancements rather than practical SE applications. However, this paper introduces an SE perspective by focusing on FM leaderboards, covering both development and operational aspects, a topic that has not yet been explored by existing SE studies. This unique angle is crucial, as it addresses the operational challenges and deployment considerations of FM leaderboards for real-world applications, an area that mainstream SE research could find highly relevant.


%Seaborn~et~al.~\cite{seaborn2015gamification} provide a comprehensive analysis of gamification from theoretical and applied perspectives, offering insights into its conceptualization, implementation, and impact on participants in various domains. 
%Additionally, Weber~et~al.~\cite{weber2019essential} offer essential guidelines for designing, performing, and interpreting high-quality benchmarking studies in computational biology to help researchers make rigorous, informative, and unbiased comparisons of different methods. 

% Barik~et~al.~\cite{barik2016perspective} offer a formal argument that gamification, as commonly applied, tends to focus narrowly on reward-based mechanics, such as points, leaderboards, and badges, while neglecting other essential game elements, such as purpose, aesthetic, and framing. 

% For example, we retain only the Multi-modal Leaderboard and exclude the OpenVLM Leaderboard, as it is an identical version released by OpenCompass\footnote{\url{https://huggingface.co/spaces/opencompass/open_vlm_leaderboard/discussions/1}}. 

% These keywords are ``benchmark'', ``dataset'', ``leaderboard'', ``foundation model'', ``large action model'', ``large AI model'', ``large audio model'', ``large audio language model'', ``large behavior model'', ``large language model'', ``large multimodal model'', ``large speech model'', ``large vision model'', ``large time series model'', ``large trajectory model'', and ``small language model''.

%\item We find that the ``unclear component'' is the most impactful type of smell, followed by the ``mismatched component'', the ``missing component'', and the ``obsolete component''. We also notice that the leaderboards suffer the most smells, followed by the participatory model and the evaluation record.

% In this paper, we present three key contributions to the ML community drawing from the findings of our study.
% \begin{itemize}[leftmargin=*]
% \end{itemize}

% Figure presents $10$ workflow patterns within the LBOps framework. Each block represents an operation (abbreviated) linked to a specific role (color-coded), as indicated in the right annotation. The arrow represents the sequence of operations in the respective workflow. The braces enclose optional operations, providing adaptability and customization to accommodate diverse evaluation requirements. Since documentation \& reporting, and inquiry \& feedback operations are intrinsic to each workflow pattern, we opt not to include them explicitly in the figure for improved clarity and conciseness. By integrating various operations and promoting seamless collaboration among stakeholders, LBOps ensures that leaderboards remain current, transparent, and adaptable to the ever-evolving landscape of ML research.

% \subsection{Evaluation Operations}

% Drawing from these operations and their variants, we have recognized $10$ evaluation workflow patterns that form the backbone of the leaderboard development process. The following section offers an in-depth exploration of the operation types and workflow patterns.



    % \item \textit{Model selection} involves choosing suitable ML models for evaluation, typically carried out by leaderboard administrators.
  % \item \textit{Inference} involves  As a pre-step before evaluation, this operation is essential for determining a model's performance, ranking, and ability to generalize beyond the training dataset.
  % \item \textit{Judgement} evaluates and compares model performance in blind testing scenarios, often integrating human preference with pairwise model comparisons. This method augments the quantitative analysis with qualitative factors, providing a well-rounded assessment of the capabilities of the models. A representative example is Chatbot Arena\footnote{\url{https://chat.lmsys.org}\label{footnote:Chatbot Arena}}.
  % \item \textit{Evaluation} examines the performance of ML models against predefined metrics to determine their position on the leaderboard. This operation plays a critical role in benchmarking models' abilities to tackle the challenges set forth by the evaluation criteria, providing insights into their strengths and areas for improvement.
  % \item \textit{Submission} involves participants who contribute their models, predictions, or evaluations through established submission channels, following specified guidelines. Adherence to the submission guidelines ensures consistency in the benchmarking process and subsequent model ranking on the leaderboards.
  % \item \textit{Submission Review} involves the verification of submissions to ensure compliance with the established criteria for further processing by leaderboard administrators. The review process is vital to maintain the credibility and quality of the leaderboards, ensuring that only eligible and high-quality submissions are integrated.
  % \item \textit{Collection} involves scraping and collecting evaluation results from multiple sources, such as academic literature and model cards. A notable example is the collaboration between PWC and Hugging Face, where PWC collects evaluations from model cards in Hugging Face\footnote{\url{https://huggingface.co/docs/hub/model-cards}\label{footnote:model card}}.
  % \item \textit{Update} involves updating the current leaderboards with new evaluation results. By regularly performing this operation, the leaderboards remain up-to-date and accurately represent the latest advances and competitive rankings among the participative models.
  % \item \textit{Release} involves the public launch of the leaderboards, inviting community participation, and fostering competition. 
  % \item \textit{Deprecation} involves the systematic removal or archiving of outdated components, such as participative models, evaluation records, leaderboards, benchmarks, and documentation. A prominent example is the ANLI\footnote{\url{https://github.com/facebookresearch/anli}\label{footnote:ANLI}} (Adversarial Natural Language Inference), which has been archived by the publishers and is no longer open to new submissions. This practice ensures that leaderboards reflect the latest research and advances in the field, fostering the development of cutting-edge models and methodologies.
  % \item \textit{Documentation \& Reporting} focus on creating, maintaining, and regularly updating comprehensive documents that describe the processes, protocols, and results pertaining to leaderboard systems. Thorough and well-organized documentation acts as a vital resource for participants, administrators, and users, encouraging transparency and facilitating easy access to relevant information.
  % \item \textit{Inquiry \& Feedback} facilitate open communication between users and leaderboard administrators, allowing the exchange of valuable input, feedback, and addressing questions or concerns related to various aspects of the leaderboard systems. Such interactions contribute to the continuous refinement of the system and promote transparency within the ML community. Different platforms offer varying levels of support for these communication mechanisms. For example, GitHub provides feedback channels through its issue reports and sometimes contact information with repository maintainers. In comparison, Hugging Face enables feedback through community discussion forums, direct contact information with repository maintainers, and accessible GitHub profiles within the application interface, if available. Moreover, PWC supports feedback only via email for users seeking assistance or clarifications. Independent platforms generally provide one or two communication channels, such as direct contact information with leaderboard administrators and associated GitHub repositories, ensuring that users can actively engage in communication or submissions to leaderboard systems while maintaining open communication with administrators.
  
%Lastly, leaderboard administrators can opt to develop their own platforms for presenting leaderboards, offering greater flexibility and tailoring them to the specific requirements and preferences of their respective communities. 
    
% These imbalances may perpetuate existing power dynamics within the field, hinder diversity and innovation, and potentially influence research priorities in favor of those with the most representation in these critical domains.

% On the other hand, we find that PWC stands out as the most prolific organization that releases leaderboards among the $234$ identified organizations, contributing to notable $43.05\%$ ($189$ out of $439$) leaderboard systems. This is followed by AI2\footnote{\url{https://leaderboard.allenai.org}\label{footnote:AI2} ($6.38\%$) and Shanghai AI Laboratory\footnote{\url{https://www.shlab.org.cn}} ($5.92\%$)}. In particular, $5.69\%$ of the leaderboard systems are released by independent contributors not affiliated with any particular organization. The Gini coefficient~\cite{gini1936measure}\footnote{Gini coefficient measures inequality, with values ranging from $0$ (representing perfect equality) to $1$ (denoting perfect inequality).} of $0.631$ underscores a high level of inequality within the distribution of leaderboard systems among release organizations, reinforcing the observation that a limited number of organizations monopolize the landscape by maintaining multiple leaderboard systems. 

% Furthermore, we conduct separate analyses for certain components of PWC and non-PWC leaderboards to account for their unique objectives, thus providing a more comprehensive and focused evaluation.

% Together, these components contribute to a robust and effective benchmark that enables meaningful and reliable performance evaluations within the specific domain. A well-designed leaderboard can significantly improve the overall user experience and encourage greater engagement within the ML community.

%To further quantify the impact of these smells, we introduce the concept of ``leaderboard smell coverage'' (LSC). Drawing inspiration from ``architectural smell coverage''~\cite{le2016relating} (ASC) in the domain of software code smell, which measures the spread of architectural smells across a leaderboard system, LSC measures the extent to which different components are affected by leaderboard smells. This metric serves as an indicator of the overall health of a leaderboard system. 

% Our study uncovers a significant gap: Only $12.98\%$ leaderboard systems provide at least one downloadable format, revealing a prevalent but overlooked tendency among ML practitioners to rely on visual comparisons over quantitative analysis for model rankings. This over-reliance on top-performing models may oversimplify the complex trade-offs involved in model selection, neglecting the potential depth of analytical insights. We advocate for a paradigm shift towards more precise and quantitative analytical methods in handling the extensive amount of evaluations within leaderboards. By adopting this approach, we can gain actionable insights into the usability of various leaderboards across different domains, ultimately enabling more informed decision-making for developers. This shift would help bridge the gap between visual comparisons and quantitative analysis, promoting a more comprehensive understanding of model performance.

%Datasets play a crucial role in determining a benchmark's relevance and representativeness within a specific domain. A task is a predefined objective or problem, such as classification, regression, and clustering, that a model is expected to solve using the provided dataset. Common examples include accuracy, precision, recall, and F1 score for classification tasks. Metrics enable a standardized way of quantifying and comparing the effectiveness of different models in tackling the benchmark's tasks. They often outline train-test splits, data preprocessing steps, and other specific requirements to ensure consistent and fair comparisons between models. It operates by thoroughly testing models against a carefully curated dataset, utilizing the benchmark's predefined metrics and a well-defined evaluation configuration to accurately measure performance. 

% Our research aims to examine leaderboard systems from three different perspectives. First, we investigate the constituent elements and building blocks that form the foundation of the reference architecture for leaderboard systems. Secondly, we investigate the processes involved in their management and maintenance (\ie, their operations). Finally, we study the various challenges and issues that arise during these operations (\ie, their smells). By investigating the reference architecture, operational patterns, and smells of leaderboard systems, we aim to equip leaderboard system developers, maintainers, and other stakeholders with empirically grounded knowledge that contributes to improving benchmarking and evaluation processes in real-world scenarios.

% To gain a comprehensive understanding of each distribution's properties and underlying patterns, we evaluate key statistical metrics, including the mean value, median value, interquartile range (IQR), and Gini coefficient. Collectively, these statistical metrics provide important insight into the statistics of each distribution. The IQR serves as an indicator of statistical dispersion, illustrating the spread of values within a dataset. The Gini coefficient~\cite{gini1936measure}, a concept borrowed from economics, measures inequality, with values ranging from $0$ (representing perfect equality) to $1$ (denoting perfect inequality). By examining the Gini coefficient, we can assess the level of concentration or dispersion within the distributions of leaderboard systems and their components, highlighting any inequalities or imbalances that may exist. 

% \textbf{Distribution of Leaderboard Systems across Release Organizations}: We find that PWC stands out as the most prolific organization that releases leaderboards among the $234$ identified organizations, contributing to notable $43.05\%$ ($189$ out of $439$) leaderboard systems. This is followed by AI2\footnote{\url{https://leaderboard.allenai.org}\label{footnote:AI2} ($6.38\%$) and Shanghai AI Laboratory\footnote{\url{https://www.shlab.org.cn}} ($5.92\%$)}. In particular, $5.69\%$ of the leaderboard systems are released by independent contributors not affiliated with any particular organization. The Gini coefficient of $0.631$ underscores a high level of inequality within the distribution of leaderboard systems among release organizations, reinforcing the observation that a limited number of organizations monopolize the landscape by maintaining multiple leaderboard systems. 

% \textbf{Distribution of Leaderboard Systems across Downloadable File Formats}: We find that only $12.98\%$ ($57$ out of $439$) leaderboard systems provide downloadable file formats for their leaderboards. This highlights a widespread, yet often disregarded, inclination among ML practitioners to favor visual comparisons over quantitative analysis when assessing model rankings. Such an overreliance on top-performing models can lead to an oversimplification of the intricate trade-offs inherent in model selection, potentially undermining the wealth of insights that could be gained through in-depth quantitative approaches. Of these downloadable file formats, \textit{CSV} (comma-separated values) proves to be the most prevalent storage format for leaderboards, accounting for $78.95\%$ ($45$ out of $57$) leaderboard systems. Other formats, including \textit{JSON} (JavaScript object notation) ($8.77\%$), \textit{XLSX} (Microsoft Excel spreadsheet) ($5.26\%$), \textit{TSV} (tab-separated values) ($3.51\%$), \textit{LATEX} (Lamport's TeX) ($3.51\%$), \textit{MD} (markdown file) ($1.75\%$), \textit{XLS} (Excel spreadsheet) ($1.75\%$), and \textit{JSONL} (JSON lines format) ($1.75\%$), are less frequently used. The notable high Gini coefficient of $0.795$ reveals a very high level of inequality in the distribution of downloadable formats in different systems. This inequality may impede efficient data sharing, collaboration, and reproducibility of results, creating barriers for practitioners who rely on specific formats for their work.

% Collectively, our analysis uncovers substantial heterogeneity in the distribution of leaderboards and their associated characteristics, highlighting the diverse landscape of ML benchmarking. In particular, \textbf{there is a substantial inequality in the distribution of leaderboards, display formats, downloadable formats, publication venues, and release organizations, as well as in the allocation of evaluation records across leaderboard systems.} However, we observe \textbf{a relatively little variation in the distribution of leaderboard systems across platforms, suggesting consistent representation in these areas.}

%On the other hand, the mean number of leaderboard systems per release organization is $3.49$, with a median value of $1$.  The IQR of $1$ highlights a narrow spread of values around the median, indicating that the number of leaderboard systems per organization is generally low for most, but increases for some, hence the high skewness. 

% \textbf{Distribution of Leaderboard Systems across Publication Venues}

% We find that $85.42\%$ ($375$ out of $439$) leaderboard systems are associated with specific publications, such as research articles, blog posts, and white papers. Of these, $61.87\%$ ($232$ out of $375$) publications have been accepted in a specific workshop, conference, magazine or journal. In particular, EMNLP\footnote{\url{https://aclanthology.org/venues/emnlp}} emerges as the conference with the highest number of accepted articles, representing $16.81\%$ ($39$ out of $232$) of those published. It is followed by NeurIPS\footnote{\url{https://neurips.cc}} ($10.78\%$) and ACL\footnote{\url{https://aclanthology.org/venues/acl}} ($9.05\%$). On the other hand, the mean number of leaderboard systems associated with different publication venues is $3.89$, while the median value is only $1$. The IQR of $1$ indicates a relatively narrow distribution of values around the median. The Gini coefficient of $0.647$ signifies a high level of inequality in the distribution of leaderboard systems associated with different publication venues.

% \subsection{Distribution of Evaluation Records across Leaderboard Systems}

% We find that HELM (Classic)\footref{footnote:HELM (Classic)} has the highest number of evaluation records up to $16,005$, followed by LMExamQA\ref{footnote:LMExamQA} ($7,096$) and Open LLM Leaderboard (GPT)\footref{footnote:Open LLM Leaderboard (GPT)} ($5,839$). On the other hand, the mean number of evaluation records in various leaderboard systems is $187.9$, with a median value of $23$. The IQR of $49$ reveals a considerable spread of values around the median, reflecting a wide variance in the number of evaluation records maintained by different systems. The Gini coefficient of $0.873$ starkly underscores this variance, indicating a very high level of inequality in the distribution of evaluation records across leaderboard systems. % The distribution underscores a significant diversity in the number of evaluation records held by leaderboard systems, with a pronounced skew towards systems with fewer records, yet with substantial variation reflecting both extremes of very few and very many records.

% Following several rounds of discourse, we identify $8$ types of leaderboard smell targeting $10$ critical components of leaderboard systems, as outlined in Section~\ref{sec:rq3-results}. 

% In this section, we compile and analyze meta-information from the collected leaderboards to examine the distribution of various types of leaderboard system and their associated characteristics. Meta-information encompasses several key aspects: leaderboard display formats across platforms, downloadable formats, participative model linkage practices, publication venues, and release organizations. By examining these factors, we aim to provide a comprehensive understanding of the current landscape of leaderboard systems and their functionalities.

% In total, Our multifaceted contributions, including a curated ML leaderboard list, enrichment of dataset profiles in PWC, and active participation in leaderboard system maintenance, exemplify our dedication to advancing best practices and promoting the evolution of leaderboard systems within the ML community. Our findings provide valuable insights for developers and researchers seeking to understand and improve current model evaluation practices. 

% Through this comprehensive analysis, we aim to reveal patterns and trends that can inform the development and optimization of leaderboard systems and ultimately enhance the benchmarking and evaluation processes in machine learning research.

% Similarly, the Video-Bench leaderboard features evaluation records with non-descriptive model names, such as ``test\_410''\footnote{\url{https://huggingface.co/spaces/LanguageBind/Video-Bench/discussions/3}}. The leaderboards released by the Allen Institute for AI\footref{footnote:Allen Institute for AI}, such as SciFact, also list models with unclear names, such as ``qr\_test0'', and descriptions marked ``to be updated''\footnote{\url{https://leaderboard.allenai.org/scifact/submission/ce0cbc2odv44t2mapeu0}}.
 
%Additionally, SuperCLUE-Code3 did not specify the detailed steps to obtain the unweighted score on its leaderboards\footnote{\url{https://github.com/CLUEbenchmark/SuperCLUE-Code3/issues/2}}. Similarly, the LLM Benchmarker Suite states that each dataset is accompanied by its respective evaluation metrics, but does not provide documentation detailing these metrics\footnote{\url{https://github.com/TheoremOne/llm-benchmarker-suite/issues/9}}. Furthermore, OpenCompass does not specify the evaluation metrics for HumanEval~\cite{chen2021evaluating} in its documentation\footnote{\url{https://github.com/open-compass/opencompass/discussions/687}}.  
 
 %The Multi-modal Modal Leaderboard's ambiguous use of ``normalized'' in MME evaluations\footnote{\url{https://github.com/open-compass/opencompass/discussions/784}}, along with benchmarks, such as ``CHIP-CDEE'', in MedBench with their scant documentation\footnote{\url{https://github.com/open-compass/opencompass/discussions/785}}, highlights a broader issue within the ML research community regarding clarity and accessibility. The omission of documentation from the LLMs Coding Leaderboard for its second split further exemplifies the gap in providing comprehensive information\footnote{\url{https://github.com/TabbyML/tabby/discussions/1368}}. The ConTextual\footnote{\url{https://huggingface.co/spaces/ucla-contextual/contextual\_leaderboard/discussions/2}} and Guerra LLM AI Leaderboards\footnote{\url{https://huggingface.co/spaces/luisrguerra/guerra-llm-ai-leaderboard/discussions/3}}\footnote{\url{https://huggingface.co/spaces/luisrguerra/guerra-llm-ai-leaderboard/discussions/2}} also struggle with ambiguity and omission in their documentation regarding evaluation datasets. Discrepancies in scenario counts are evident in both HELM (Classic), between its main page and documentation\footnote{\url{https://github.com/stanford-crfm/helm/issues/2028}}\footnote{\url{https://github.com/stanford-crfm/helm/issues/2358}}, and in HELM (Instruct), where the counts for the ``Anthropic Red Team'' benchmark diverge between official documents and blog posts\footnote{\url{https://github.com/stanford-crfm/helm/issues/2441}}.

% Additionally, HELM (Classic) fails to define the ``prompt\_num\_line'' parameter in its copyright code benchmark specification\footnote{\url{https://github.com/stanford-crfm/helm/issues/2350}}. Moreover, the evaluation details are missing from the MOE LLM GPU-Poor Leaderboard\footnote{\url{https://huggingface.co/spaces/PingAndPasquale/MOE-LLM-GPU-Poor-Leaderboard/discussions/2}}.

%Both the overall leaderboard\footnote{\url{https://github.com/Q-Future/Q-Bench/issues/11}} and the A2 leaderboard for Chinese\footnote{\url{https://github.com/Q-Future/Chinese-Q-Bench/issues/2}} of Q-Bench exhibit misalignment problems. % Furthermore,  A similar crash issue is observed on the Open LLM Leaderboard (GPT)\footnote{\url{https://huggingface.co/spaces/gsaivinay/open\_llm\_leaderboard/discussions/5}}. \\

% The ANLI repository\footref{footnote:ANLI} has been archived, making its submission channels obsolete. 

%KoLA has discontinued support for week-level queries in its leaderboard search panel, and users can access leaderboards only on a seasonal basis\footnote{\url{https://github.com/THU-KEG/KoLA/issues/3}}.
    
% There are identical evaluation records in multiple scenarios on the HEIM leaderboard\footnote{\url{https://github.com/stanford-crfm/helm/issues/2176}}

% LLMEval now exclusively adopts the most recent benchmark, LLMEval-3\footnote{\url{https://github.com/llmeval/llmeval-2}\label{footnote:LLMEval-3}}, for the evaluation of models. This update makes its predecessors, LLMEval-1\footnote{\url{https://github.com/llmeval/llmeval-1}\label{footnote:LLMEval-1}} and LLMEval-2\footnote{\url{https://github.com/llmeval/llmeval-2}\label{footnote:LLMEval-2}}, obsolete. Similarly,  Furthermore, Open Dutch LLM Evaluation Leaderboard\footnote{\url{https://huggingface.co/spaces/BramVanroy/open_dutch_llm_leaderboard}}. Several leaderboards, including C-Eval\footnote{\url{https://github.com/hkust-nlp/ceval/issues/76}}, LAiW\footnote{\url{https://huggingface.co/spaces/daishen/SCULAiW/discussions/1}}, Xiezhi\footnote{\url{https://github.com/MikeGu721/XiezhiBenchmark/issues/6}}, and L-Eval\footnote{\url{https://github.com/OpenLMLab/LEval/issues/10}}, face issues of desynchronization with their latest evaluation results.

% Although the original HELM paper~\cite{bommasani2023holistic} includes WikiText-103~\cite{merity2016pointer} and NewsQA~\cite{trischler2016newsqa} in its supported scenarios, these benchmarks are not available for evaluation on current leaderboards\footnote{\url{https://github.com/stanford-crfm/helm/issues/2239}}. % Furthermore,  Similarly, the ``junior-dev'' dataset is deprecated in the CanAiCode Leaderboard\footnote{\url{https://huggingface.co/spaces/mike-ravkine/can-ai-code-results/discussions/7}}.
    
% Users encounter difficulties when trying to create new accounts or log into existing ones on the KoLA\footnote{\url{https://github.com/THU-KEG/KoLA/issues/9}} and LawBench\footnote{\url{https://github.com/open-compass/LawBench/issues/11}} platforms, respectively. Open ITA LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/FinancialSupport/open_ita_llm_leaderboard/discussions/4}}.
 
% The audio leaderboards are not accessible in FlagEval\footnote{\url{https://github.com/FlagOpen/FlagEval/issues/37}}. Furthermore, an event of restricting network access for external users was reported in both Safety Prompts\footnote{\url{https://github.com/thu-coai/Safety-Prompts/issues/18}} and OCRBench\footnote{\url{https://github.com/Yuliang-Liu/MultimodalOCR/issues/23}}.

% A comparable situation occurs with the WHOOP! leaderboard\footnote{\url{https://github.com/whoops-benchmark/whoops-benchmark.github.io/issues/1}}.

% This cap significantly limits the scope of the analysis, as it prevents access to all evaluations from the dashboard. Similarly, SuperCLUE experienced an issue in which GPT-4 Turbo\footnote{\url{https://platform.openai.com/docs/models/gpt-4-and-gpt-4-turbo}} was accidentally excluded from its evaluation records in its December release\footnote{\url{https://github.com/CLUEbenchmark/SuperCLUE/issues/41}}. Additionally, on the LLM Safety Leaderboard, selecting specific column options can cause certain evaluation records to disappear from the display, and these records do not reappear even after the options are deselected\footnote{\url{https://huggingface.co/spaces/AI-Secure/llm-trustworthy-leaderboard/discussions/5}}.
 
% \item \textit{Evaluation Script}: The OpenEval GitHub repository is inaccessible\footnote{\url{https://github.com/tjunlp-lab/Awesome-LLMs-Evaluation-Papers/issues/24}}.
    
% Similarly, the KoLA submission portal lacks a configuration template for the participatory models\footnote{\url{https://github.com/THU-KEG/KoLA/issues/16}}.

% Participatory models were not mentioned on the Leaderboard\footnote{\url{https://huggingface.co/spaces/mteb-pt/Leaderboard/discussions/1}}. Furthermore, the model in the second row is not specified on the CALLHOME speaker verification leaderboard\footnote{\url{https://paperswithcode.com/sota/speaker-verification-on-callhome}}.
    
% Similarly, the ``intellectual ability'' leaderboard is missing from OpenEval\footnote{\url{https://github.com/tjunlp-lab/Awesome-LLMs-Evaluation-Papers/issues/27}}.  The same issue had occurred on the KoLA leaderboards since the beginning of the $2024$\footnote{\url{https://github.com/THU-KEG/KoLA/issues/18}} calendar year. Similarly, there are many empty leaderboards hosted on Paper~With~Code\footnote{\url{https://paperswithcode.com/sota/instance-segmentation-on-cityscapes}}\footnote{\url{https://paperswithcode.com/sota/reinforcement-learning-on-seals-ant-v0-1}}. This issue also happened with the Ko Chatbot Arena Leaderboard\footnote{\url{https://huggingface.co/spaces/instructkr/ko-chatbot-arena-leaderboard/discussions/4}}. Occasionally, OpenCompass leaderboards are missing because they are not in sync with their respective hosting platforms\footnote{\url{https://huggingface.co/spaces/opencompass/opencompass-llm-leaderboard/discussions/3}}.
 
%OpenEval lists two metrics for specific benchmarks, but presents only evaluation records for one\footnote{\url{https://github.com/tjunlp-lab/Awesome-LLMs-Evaluation-Papers/issues/21}}. Similarly, the LLMEval-3 framework identifies 13 evaluation scenarios, but current leaderboards show results for only 11 of these\footnote{\url{https://github.com/llmeval/llmeval-3/issues/1}}. Moreover, MMLU evaluations are not found on the MY Malay LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/mesolitica/malay-llm-leaderboard/discussions/3}}. Additionally, the GAOKAO-Bench leaderboard showed missing submissions for ``fill-in-the-blank'' and ``open-ended'' questions\footnote{\url{https://github.com/OpenLMLab/GAOKAO-Bench/issues/25}}. 
    
% Similarly, the evaluation details are missing from the M3DBench documentation\footnote{\url{https://github.com/OpenM3D/M3DBench/issues/2}}.
    
%HELM (CLassic)\ref{footnote:HELM (Classic)} claims to support a wide range of scenarios, including BillSum~\cite{kornilova-eidelman-2019-billsum}, EurLexSum~\cite{aumiller2022eur}, LegalBench~\cite{guha2023legalbench}, MultiLexSum~\cite{shen2022multi}, Numerical reasoning~\cite{bommasani2023holistic}, and WMT 2014~\cite{bojar2014findings}. However, these benchmarks are conspicuously absent from HELM (Classic)\footnote{\url{https://github.com/stanford-crfm/helm/issues/2062}}. Moreover, some datasets, such as WGlaw, are missing from the OpenEval leaderboards\footnote{\url{https://github.com/tjunlp-lab/Awesome-LLMs-Evaluation-Papers/issues/14}}. Similarly,  Furthermore, some 3d datasets, such as ScanNet~\cite{dai2017scannet}, are missing from the ChEF leaderboards\footnote{\url{https://github.com/OpenGVLab/LAMM/issues/64}}. Furthermore, despite support claims, benchmarks such as ScienceQA~\cite{saikh2022scienceqa} and COCO Captions~\cite{chen2015microsoft}, are absent from the OpenVLM Leaderboard\footnote{\url{https://huggingface.co/spaces/opencompass/open_vlm_leaderboard/discussions/3}}\footnote{\url{https://huggingface.co/spaces/opencompass/open_vlm_leaderboard/discussions/4}}\footnote{\url{https://huggingface.co/spaces/opencompass/open_vlm_leaderboard/discussions/5}}.
    
    % The evaluation configuration in LLM-Leaderboard deviates from the original package's\footnote{\url{https://github.com/LudwigStumpp/llm-leaderboard/issues/9}}. 

% FlagEval's English choice QA task documentation mentions HellaSwag~\cite{zellers2019hellaswag} and OpenBookQA~\cite{mihaylov2018can} as evaluation benchmarks, but the evaluations actually use BoolQ~\cite{clark2019boolq} and TruthfulQA~\cite{lin2021truthfulqa} instead\footnote{\url{https://github.com/FlagOpen/FlagEval/issues/35}}. Additionally, the ``valid parentheses'' task is missing from the BIG-Bench task list\footnote{\url{https://github.com/google/BIG-bench/issues/983}}. There is also an inconsistency in the name of the evaluation dataset for MGSM8KInstruct compared to the dataset that was actually used\footnote{\url{https://github.com/microsoft/MathOctopus/issues/7}}. Lastly, the AI Model Rankings leaderboard reported a discrepancy between its claim and the benchmark dataset it used\footnote{\url{https://huggingface.co/spaces/CathieDaDa/LLM_leaderboard/discussions/2}}. Open ITA LLM Leaderboard: https://huggingface.co/spaces/FinancialSupport/open_ita_llm_leaderboard/discussions/7

% By making the evaluation process more precise, we can significantly improve the reliability, fairness, and overall effectiveness of ML model assessments, driving innovation and growth across the entire field of machine learning. %This oversight not only points to a significant gap in current methodology, but also marks a fertile ground for interdisciplinary exploration. 

% LLMonitor claims that its evaluation dataset changes weekly. However, evidence suggests that the evaluation prompts have remained unchanged for several months\footnote{\url{https://github.com/lunary-ai/llm-benchmarks/issues/3}}. Details of the evaluation record are absent from the page redirected by LLMonitor\footnote{\url{https://github.com/lunary-ai/llm-benchmarks/issues/4}}.

%For instance, metric-centric leaderboards focus on evaluating and comparing the effectiveness of various evaluation metrics themselves, offering a meta-level insight into how we assess model performance. This could reveal biases or inefficiencies in current evaluation practices, potentially leading to more robust and fair measures of model capabilities. 

% \paragraph{Variability in LBOps Workflow}: We encourage researchers to document and share the unique operational workflows developed, fostering innovation and collaboration in the development of leaderboard systems. Our findings reveal various operational practices among leaderboard systems, characterized by seven distinct evaluation workflows. By sharing these practices, developers can apply different operational workflows to meet the unique needs of leaderboard systems, enhancing system transparency, fairness, and reproducibility.

% \subsection{Background}

% A leaderboard is a structured ranking system that displays and juxtaposes the performance, achievements, or scores of individuals or teams within a particular domain or activity. This system not only acts as a visual marker of progress and competitive spirit, but also serves as a dynamic tableau that highlights the relative standings of participants based on meticulously defined criteria. These criteria might range from points accrued, the expediency of task completion, to the attainment of various levels or milestones. Ubiquitous across a multitude of spheres, spanning video games, sports tournaments, educational frameworks, and corporate performance indicators, leaderboards embody a quintessential element of gamification that translates real-world activities into engaging, game-like experiences~\cite{hamari2014does}.

% The utility of leaderboards extends beyond mere ranking. They are powerful tools for motivation, creating an environment in which participants are encouraged to improve their performance and rise in the ranking. This motivational capacity is deeply rooted in the psychological principles of competition and achievement recognition, which are crucial in driving human behavior toward achievement of goals~\cite{deci2000and}. By allowing participants to visualize their position relative to peers, leaderboards catalyze a competitive yet collaborative ethos, encouraging individuals to push their boundaries and strive for excellence.

% Moreover, leaderboards offer a transparent mechanism for the acknowledgment of top performers, thus fostering a culture of meritocracy where excellence is recognized and rewarded. In educational settings, for example, they can significantly increase student participation and learning outcomes by integrating a competitive layer that resonates with the intrinsic motivation of learners~\cite{dichev2017gamifying}. In the corporate arena, leaderboards are instrumental in driving salesforce productivity, enhancing employee engagement, and catalyzing performance improvements by leveraging competitive dynamics~\cite{bunchball2010gamification}.

% In conclusion, leaderboards are not merely hierarchical ranking structures, but complex mechanisms that leverage psychological principles to foster competition, achievement, and motivation in various domains. Their implementation, when thoughtfully executed, can significantly enhance the engagement, performance, and overall experience of participants, making them a cornerstone in the design of competitive and collaborative environments.

% \begin{itemize}
% \item \textit{Participatory Model}: The models specifically evaluated in the leaderboard.
% \item \textit{Evaluation Dataset}: The benchmark datasets utilized for leaderboard evaluations.
% \item \textit{Evaluation Metric}: The metric used to assess performance on the leaderboard.
% \item \textit{Evaluation Record}: The performance records displayed on the leaderboard.
% \item \textit{Evaluation Report}: The comprehensive report detailing the evaluations conducted for the leaderboard.
% \item \textit{evaluation configuration}: The approach or methodology used for the evaluations on the leaderboard.
% \item \textit{Submission Channel}: The details of the submissions made for evaluation on the leaderboard.
% \item \textit{Leaderboard}: The current standing or condition of the leaderboard.
% \end{itemize}
% Subsequently, we detail each smell, including its type, category, definition, and illustrative examples from our dataset.
% \item \textit{Evaluation Portal}: The login portal for the leaderboard evaluation.
% \item \textit{Evaluation Script}: The script for the evaluation framework used by the leaderboard.

    % \begin{itemize}
    %     \item \emph{Regular table}: Regular tables have a straightforward layout, focusing primarily on rows of evaluation records. A representative example is the AlpacaEval leaderboard\footref{footnote:AlpacaEval}.
    %     \item \emph{Sortable table}: Sortable tables allow users to reorder rows based on specific column criteria, enhancing interactivity. A representative example is the Open LLM Leaderboard.
    %     \item \emph{Table screenshot}: Table screenshots are static image captures of regular tables, often from PDF reports. A representative example is the Xiezhi leaderboard.
    % \end{itemize}
    % Similarly, the figures are diversified into several types to suit different data visualization needs:
    % \begin{itemize}
    %     \item \emph{Bar chart}: Bar charts use vertical or horizontal bars to represent data quantities, facilitating easy comparison across categories. A representative example is the Coding LLMs Leaderboard.
    %     \item \emph{Box plot}: Box plots offer a visual summary of the data distribution and variance, which is useful for statistical analyses. A representative example is the ``throughput variance'' leaderboard in the Models Leaderboard.
    %     \item \emph{Heat map}: Heat maps show the data density or value levels through color variations. A representative example is the ``action category distribution'' leaderboard in Do-Not-Answer.
    %     \item \emph{Line chart}: Line charts connect data points with lines, suitable for showing trends over time. A representative example is the ``throughput, over time'' leaderboard in the Models Leaderboard.
    %     \item \emph{Pie chart}: Pie charts illustrate proportional contributions within a whole. A representative example is the `tool-use error distribution on test set'' leaderboard in TravelPlanner.
    %     \item \emph{Radar chart}: Radar charts display multivariate data on a two-dimensional plot, ideal for comparing multiple entities with various features. A representative example is the ``model capabilities'' leaderboard in the Nexus Function Calling Leaderboard.
    %     \item \emph{Scatter plot}: Scatter plots utilize Cartesian coordinates to visualize the relationship between two variables. Representative examples include the ``over time'' series leaderboards, which are prominently displayed alongside sortable table leaderboards in Papers With Code.
    %     \item \emph{Sortable bar chart}: Sortable bar charts are dynamic bar charts that allow reordering based on axis criteria, enhancing the data interaction with users. A representative example is the `LLMs' ability to leverage natural language feedback'' leaderboard in MINT.
    % \end{itemize}
    % It is essential to recognize that a leaderboard system can feature various leaderboard formats, sometimes using different sets of evaluation results. For example, at the Allen Institute for AI\footnote{\url{https://leaderboard.allenai.org}\label{footnote:Allen Institute for AI}}, each leaderboard is presented in two distinct formats: sortable tables and scatter plots. This variety ensures that users can interact with and interpret the evaluation data in multiple ways, catering to different preferences and analytical needs. 


    % Each record requires at least one model name alongside its evaluation result, ensuring that every entry contributes the necessary information to the leaderboard. Furthermore, a record could include a vast array of context information, thereby enriching the leaderboard with detailed insights into each model's performance.

    % \begin{itemize}
    %     \item \emph{Evaluation dataset}: At the core of any benchmark is the evaluation dataset, a meticulously curated compilation of data designed to test models under conditions that mimic real-world scenarios or specialized synthetic settings. These datasets encompass a wide spectrum of data samples, each selected to challenge and reveal the nuances of model performance in a variety of situations. The diversity and relevance of these datasets are crucial, as they directly influence the benchmark's ability to evaluate models effectively and fairly.
    %     \item \emph{Evaluation metric}: Evaluation metrics are standardized yardsticks to measure and compare the performance of ML models. They are chosen for their relevance to the intended application of the model, providing a clear and consistent means of evaluating the effectiveness, reliability, and suitability of the task. Through these metrics, stakeholders can make informed decisions about model selection, refinement, and advancement, grounded in a framework that quantifies achievement in relation to the benchmark's goals.
    %     \item \emph{Evaluation strategy}:  The strategy specifies the conditions under which evaluations are performed, including train-test splits, data preprocessing techniques, and prompt engineering approaches, to ensure a standardized, reproducible, and fair comparison among various models or algorithms.
    % \end{itemize}
    
    % MLESOps encompasses the methodologies, tools, and practices vital to the effective management, operation, and evolution of MLES. By exploring MLESOps, we emphasize the importance of addressing the intricate processes involved in designing, configuring, and maintaining ML leaderboards. This includes managing leaderboard presentation, evaluation submissions, documenation \& reports, and ensuring their reliability, fairness, and relevance within the competitive landscape of ML models.

% \item \emph{Evaluation Strategy}: This encompasses the comprehensive methodology and systematic arrangement devised to assess model performance. It details the frameworks, criteria, and processes used to evaluate and benchmark the effectiveness, efficiency, and accuracy of models. The strategy is designed to ensure a thorough and objective analysis of the model capabilities, aligning the evaluation methods with specific goals and performance measurement standards.
% \item \emph{Organization strategy}: This refers to the systematic approach and structural arrangement used to organize evaluations in a user-friendly presentation format. It encompasses the strategies and techniques used to categorize, display, and interpret evaluation results, ensuring that they are accessible and comprehensible to users. This aspect focuses on optimizing the user experience by facilitating easy navigation and interpretation of the evaluation results.

% We begin our analysis by addressing the four research questions in a systematic but heuristic manner. We spend time checking the collected LES on by one in terms of their leaderboards, documentation, and report, if any. In particular, we record the meta information on the characteristics of LES, including their components, evaluation workflow, host platform, etc.. Whenever we encounter any concerns or questions, we initiate discussion in their respective repository via issue tracker. We raise about $350$ issues on GitHub and $150$ discussions on Hugging~Face to confirm our understanding of their LES in terms of $10$ major asssets: participatory models, evaluation codebase, benchmark datasets, evaluation metrics, evaluation results, evaluation reports, evaluation strategies, submission details, and leaderboards. Of these, $275$ of GitHub and $45$ get reponses from the respository maintainers. Meanwhile, the first and second authors periodically discuss the reponses from the issue trackers. We categorize our findings via ground theory in software engineering and refine our terminology through multiple rounds of negotiation. In case there is any contraversies between the two authors, a third author would join and make a judgement to finalize the decision. This negotiated agreement approach along with the verifiable issue trackers add credibitlity to our analysis in terms of our findings.

% It is essential that each leaderboard system incorporates at least one presentation format to ensure effective information communication. 
 
% Starting with an exploration of the development lifecycle of leaderboards, we scrutinize the collected leaderboard systems based on the elements outlined in Section~\ref{sec:background}. This sequential approach allows us to progressively build upon our findings and deepen our understanding of the complexities inherent in LESOps. Next, we investigate the organization strategies adopted by leaderboard administrators, highlighting their rationale for aggregating evaluation results into multiple leaderboards. Furthermore, we examine the distribution patterns of the assets in the leaderboard systems, including most of , which sets the stage for an in-depth correlation analysis based on these patterns. Finally, we summarizes the operational smells identified through the observation of LESOps in various leaderboard systems. We synthesize these findings into actionable insights, providing a foundation for future improvements in the design, implementation, and maintenance of leaderboard systems to ensure transparency, reproducibility, and fairness in model evaluation.

% \item We exclude leaderboards that accommodate at most one participatory model. For example, TOFU leaderboard\footnote{\url{https://huggingface.co/spaces/locuslab/tofu_leaderboard}} only benchmark on GPT-4 model, and Qwen-72B in C-Eval\footnote{\url{https://cevalbenchmark.com/static/model.html?method=Qwen-72B}} and those found in the . This approach ensures that the selected leaderboards serve designated comparative purposes.
    
% \item We exclude leaderboards that serve primarily as promotional platforms for new models, as these leaderboards often feature models that are excessively fine-tuned to their respective benchmarks, potentially compromising the objectivity and generalizability of model evaluations. Examples include MAmmoTH\footnote{\url{https://github.com/tiger-ai-lab/mammoth}}, Humback\footnote{\url{https://github.com/Spico197/Humback}}, MPT-7B\footnote{\url{https://www.databricks.com/blog/mpt-7b}}, LAION-5B\footnote{\url{https://laion.ai/blog/laion-5b}}, MetaMath\footnote{\url{https://github.com/meta-math/MetaMath}}, LongForm\footnote{\url{https://github.com/akoksal/LongForm}}, MusicQA\footnote{\url{https://github.com/crypto-code/mu-llama}}, Video-ChatGPT\footnote{\url{https://github.com/mbzuai-oryx/Video-ChatGPT}}, Youku-mPLUG\footnote{\url{https://github.com/X-PLUG/Youku-mPLUG}}, Xwin-LM\footnote{\url{https://github.com/Xwin-LM/Xwin-LM}}, , and WizardLM\footnote{\url{https://github.com/nlpxucan/wizardlm}}.
    
%For example, within the data panel of the LMExamQA leaderboard\footnote{\url{https://lmexam.com}\label{footnote:LMExamQA}}, users can evaluate candidate models by randomly selecting three samples from the test dataset.
% \begin{enumerate}[label=\Alph*.]
    %     \item \textit{}: This allows leaderboard administrators to access the capabilities of the trained model for a specific task. A representative example is the Open LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/gsaivinay/open_llm_leaderboard}\label{footnote:Open LLM Leaderboard}}.
    %     \item \textit{Prediction results}: These are the outputs generated by the model for a given task. A representative example is LLMEval\footnote{\url{https://github.com/llmeval}\label{footnote:LLMEval}}.
    %     \item \textit{Evaluation results}: These are the performance metrics of the model on the specified task. A representative example is LLM-Leaderboard\footnote{\url{https://github.com/LudwigStumpp/llm-leaderboard}\label{footnote:LLM-Leaderboard}}.
    % \end{enumerate}
    

% This approach guarantees a thorough and varied compilation of evaluation resources, allowing a detailed and up-to-date understanding of the evolving dynamics and progressions of LES.
%Then, we create a list of keywords associated with foundation models or evaluation by collaborative discussion among authors. These terms include ``benchmark'', ``dataset'', ``leaderboard'', ``foundation model'', ``large action model'', ``large audio model'', ``large audio language model'', ``large language model'', ``large multimodal model'', ``large speech model'', ``large vision model'', ``large time series model'', ``large trajectory model'', and ``small language model''. For GitHub searches, we prefix ``awesome'' to each aforementioned keyword to retrieve awesome lists that collage resources in FM evaluation. In Google~Scholar, we suffix ``review'', ``survey'', and ``study'', respectively, to each of the aforementioned keywords to search for the literature review on FM evaluation. Given the large volume of literature retrieved, we limit our examination to the first $20$ pages for each search term. This systematic approach to keyword selection and tailored search strategies across different venues enables us to efficiently navigate and distill the vast landscape of literature pertaining to FM evaluation. Table~\ref{tab:retrieved literature} shows the comprehensive compilation of literature from different sources after this process. % drawing inspiration from the rich variety of terms identified in the existing multivocal literature and insights from experts in the field %This strategy allows us to identify and analyze repositories that have garnered at least 100 stars, as suggested by Borges~et~al.~\cite{borges2018s}. In Hugging~Face~Spaces, we gather all the needed information from hosted leaderboards directly. 

% Our research aims to systematically explore the operational dynamics within leaderboard systems, with a focus on FM leaderboards. By investigating four core research questions, our study aims to (1) delineate how the core practices of LBOps vary across different hosting platforms to understand their adaptation to meet diverse community needs and task requirements; (2) examine how leaderboard publishers organize evaluation records into multiple leaderboard splits; (3) identify distribution patterns of leaderboards along with their assets to assess their transparency, accessibility, and usability; and (3) uncover the types of smell within these leaderboards to highlight the complexity of evaluating FMs. The objective of this research is not only to provide insight to researchers and developers on selecting the most suitable platforms and practices to publish or participate in leaderboards, but also to shed light on best practices that can enhance transparency, fairness, and reproducibility in the evaluation of ML models. In doing so, our goal is to contribute to the advancement of the field by encouraging innovation in leaderboard design and implementation, ultimately fostering the development of more robust, equitable, and efficient models. This study aims to reach a diverse audience, including FM researchers, developers, and testers in the ML community, offering them a roadmap to improve the credibility and effectiveness of FM leaderboards as tools to benchmark progress and advance the state-of-the-art in FM research and applications.

 %For SE researchers, it is imperative to prioritize creating adaptive, intuitive environment management systems that integrate with various ML tools and platforms throughout the ML development lifecycle. SE educators should focus on enriching the curriculum in areas such as software environment and dependency management, as well as model deployment and serving, while also promoting the use of tool-specific forums for real-time, hands-on problem solving in ML asset management. Application developers need to improve their expertise in crucial areas such as software environment and dependency management to ensure seamless ML application development. Lastly, tool developers should pay attention to enhancing features tied to environment management and model deployment, making sure that tools are user-friendly, interoperable across platforms, and paired with comprehensive documentation.
%Lastly, we find that problem inquiries appear more frequently than knowledge inquiries related to machine learning asset management. Macro-topics concerning visualization and user interface, data preparation and development, and model deployment and serving show the highest unsolved rates. Meanwhile, topics on experiment tracking, source code tracking, and logs and monitoring take the longest median time to address. 

% We find that different platforms perform differently even for the same operations. Thus, in the following parts, we conduct a detailed comparative analysis of LBOps on selected leaderboard hosting platforms: GitHub, Hugging Face Spaces, Papers With Code, and independent platforms as a whole. Our comparison focuses on several key operations: creation

%Papers~With~Code stands out as the leading release entity among the 162 organizations featured in the leaderboards, contributing to $25.18\%$ ($137$) of these leaderboards.  It is important to note that while Papers~With~Code serves as a key leaderboard publisher, the actual submission of evaluation results is a collaborative effort involving users from both Papers~With~Code and Hugging~Face~Spaces. Thus, Papers~With~Code acts as a facilitator for release rather than directly contributing to the evaluations. Importantly, we exclude Papers~With~Code from our analysis due to its reliance on user-contributed leaderboards. The anonymity or lack of clear affiliation of these contributors makes it difficult to accurately depict the release organization, which introduces potential biases in our analysis. However, we acknowledge exceptions such as HotpotQA\footnote{\url{https://paperswithcode.com/sota/question-answering-on-hotpotqa}\label{footnote:HotpotQA}} and MTEB\footref{footnote:MTEB}, whose leaderboards on Papers~With~Code mirror those hosted on original platforms. In such cases, we include these specific leaderboards in our analysis to maintain consistency between our data sources, ensuring a comprehensive and unbiased overview.

% \subsection{Distribution of Leaderboards across Submission Artifacts}: 

% We find that \textbf{evaluation results are the most prevalent submission artifact, represented in the $66.03\%$ ($173$ out of $262$) leaderboard systems. This is followed by prediction results ($20.99\%$) and model repositories ($2.67\%$).} Figure~\ref{fig:submission artifact distribution} illustrates the distribution of leaderboards in different submission artifacts. In particular, a minority of $13$ ($4.96\%$) leaderboards, marked in ``Unknown'', do not specify the artifacts required for user submissions, indicating a lack of clarity in the submission guidelines for these instances. The mean number of leaderboards per submission artifact is approximately $49.56$, suggesting a relatively high average count within the dataset. However, the significant disparity between the mean and the median, which is $15$, along with a mode of $1$, highlights a distribution characteristic in which most submission artifacts are associated with a single leaderboard. This discrepancy suggests that while most artifacts are linked to one leaderboard, a small number of artifacts are associated with a considerably larger number of leaderboards, significantly inflating the average. The standard deviation of $63.61$ indicates a high level of variation within the dataset, indicating substantial differences in the number of leaderboards associated with different submission artifacts. Furthermore, the Gini coefficient of $0.702$ underscores a high degree of inequality within the distribution, which means that the leaderboards are highly concentrated among a few submission artifacts. This analysis reveals a skewed distribution, where a vast majority of submission artifacts have minimal association, while a select few are linked to a large number of leaderboards, leading to a pronounced uneven distribution of leaderboards across submission artifacts.



% Our study aims to fill the aforementioned research gap by investigating the operational dynamics, organization structures, and inherent smells encountered in the development lifecycle of leaderboard-oriented evaluation systems (\ie, leaderboard system). In the course of our investigation, we have identified a novel area within the domain of leaderboard systems, which we term \textbf{leaderboard-oriented evaluation operations} (LBOps). This concept emerges from our understanding that there exists a comprehensive workflow throughout the entire development lifecycle of leaderboard systems. LBOps encompasses the methodologies, tools, and practices that are essential for the efficient management, operation, and evolution of these systems. This new discipline draws attention to the intricate processes behind the scenes, from the initial design and setup of leaderboards to the ongoing management of submissions and the dynamic updating of rankings. It also highlights the need for systematic approaches to handle the complexities involved in leaderboard systems, ensuring their reliability, fairness, and relevance in the competitive landscape of machine learning. By acknowledging and formalizing LBOps, we aim to pave the way for more sophisticated and effective leaderboard systems that can adapt to the rapidly evolving demands of machine learning research and development. During our study, we have contributed more than $200$ new benchmark profiles in Papers~With~Code\footnote{\url{https://paperswithcode.com}\label{footnote:pwc}}. We also create an awesome list for ML models on GitHub\footnote{\url{https://github.com/zhimin-z/awesome-machine-learning-leaderboard}}. To our knowledge, our study is the first to systematically investigate the operations and characteristics of FM leaderboards.

% why practitioners choose to organize the evaluation records might be multiple reasons such as https://github.com/CLUEbenchmark/SuperCLUE-Code3/issues/1

% \subsubsection{Retirement}

% After meeting specific criteria, administrators would remove the deprecated leaderboards from the platforms. For example, AlpacaEval 2.0, launched on \date{Jan 9, 2024}, represents an upgrade driven by the need for enhanced features, such as the adoption of GPT-4 as a baseline, the introduction of prompt tuning, precomputed leaderboards, a new annotator selection, website improvements for user experience, and the potential inclusion of new models and evaluation metrics, thus replacing AlpacaEval\footnote{\url{https://github.com/tatsu-lab/alpaca_eval/issues/187}}.

% MVBench~\cite{li2023mvbench} is a benchmark for evaluating multi-modal video understanding for multi-modal LLMs. It organizes its evaluation records into $20$ leaderboard splits\footnote{\url{https://github.com/OpenGVLab/Ask-Anything/tree/main/video_chat2}\label{footnote:MVBench}} based on temporal-related video tasks, such as ``action sequence'', ``counterfactual inference''.
    

% \subsubsection{Review}

% \zhimin{this section discusses review operations in terms of host platforms}
% Examining review mechanisms across different platforms uncovers considerable obstacles, primarily resulting from the lack of comprehensive documentation on their processes. Consequently, this limitation restricts our discussion to a select number of examples for each hosting platform. On GitHub, there are noticeable inconsistencies in the evaluation records for the performance of the Chinchilla-70b~\cite{hoffmann2022training} model in the MMLU few-shot task, as reported by the LLM-Leaderboard\footnote{\url{https://github.com/LudwigStumpp/llm-leaderboard/issues/10}}. 

% In Papers~With~Code, a notable discrepancy is the incorrect labeling of a leaderboard as ``Image Classification on HumanEval''\footnote{\url{https://paperswithcode.com/sota/image-classification-on-humaneval}}. In independent platforms, such as the Allen Institute for AI, a strict curation policy is prominently declared for leaderboard evaluation results. However, issues such as unintuitive model names and incomplete evaluation-specific documentation persist. For example, the submission record  on SciFact .

% Hugging~Face~Spaces is a cloud-based collaboration platform that enables users   Papers~With~Code facilitates the development of leaderboards through three primary methods: ``evaluation result'', ``model card'', and ``leaderboard''.
% \begin{itemize}
%     \item \textit{Evaluation result}: This approach allows users to directly input evaluation results into a new leaderboard from the benchmark's profile page. It simplifies the process of sharing and comparing the performance of the models. 
%     \item \textit{Model card}: By detailing the results of the model evaluation in the YAML metadata of a model card, users ensure that their contributions adhere to the specification of the Papers~With~Code model index\footnote{\url{https://huggingface.co/docs/hub/model-cards}}. This method ensures that the results are systematically indexed and easily discoverable on the appropriate leaderboards.
%     \item \textit{Leaderboard}: Papers~With~Code has expanded its functionality to include integration with ongoing competition leaderboards via EvalAI\footnote{\url{https://twitter.com/eval_ai/status/1341091250544521231}}. This facilitates a dynamic and up-to-date reflection of model standings in real-time competitions. For further information, refer to EvalAI's announcement here.
% \end{itemize}
% Furthermore, the leaderboards adhere to a consistent format, This standardized template ensures uniformity while allowing the inclusion of additional metrics relevant to the evaluation, thus accommodating a broad spectrum of evaluation criteria. 

%  Based on these user selections, the system produces provisional leaderboards in real time.

%The intricacies of leaderboard provisioning and organization are elaborated on in Section~\ref{TODO}, providing a deeper dive into the structural dynamics at play.
 
 % We focus exclusively on model-centric leaderboards, which prioritize the evaluation of the model's performance over other factors. This approach intentionally bypasses team-centric and data-centric leaderboards. On the one hand, team-centric leaderboards, exemplified by platforms, such as EvalAI\footnote{\url{https://eval.ai}} and Kaggle\footnote{\url{https://www.kaggle.com/competitions}}, emphasize team performance, presenting contextual information related to teams. On the other hand, dataset-centric leaderboards, such as those found in , highlight performance metrics related to specific datasets, offering dataset names and related context information rather than details on model performance. Our rationale for this focus comes from two main considerations. First, our research interest is primarily in the evaluation mechanisms of the models themselves, rather than in the collaborative efforts of teams or the characteristics of datasets that could influence these outcomes. Second, distinguishing whether leaderboards evaluate foundation models poses significant challenges, necessitating a more concentrated focus to ensure the clarity and relevance of our analysis.
 %We notice that some results of the leaderboards\footnote{\url{https://paperswithcode.com/sota/image-captioning-on-nocaps-in-domain}} are obtained through a collaboration between PWC and EvalAI\footnote{\url{https://twitter.com/eval_ai/status/1341091250544521231}}. Despite this partnership, we classify these leaderboards as Workflow Pattern~$7$ since our analysis reveals that all EvalAI results are submittable, editable, and removable, mirroring standard evaluation records. Furthermore, these evaluations are combined with user-submitted results, suggesting a closer association with user-submission workflows (Pattern~$7$) rather than leaderboard administrator collection workflows (Pattern~$8$).
 
% as delineated in Figure~\ref{fig:LBOps workflow}. This framework begins with the aggregation of models, benchmarks, and evaluation harnesses. Subsequently, a model is evaluated against these benchmarks using a designated harness to produce evaluation records. This procedure can be executed through various methodologies, as described in the following.
% \begin{itemize}
% \item \textit{Direct evaluation by administrators}: Leaderboard administrators directly assess models or inference APIs using reference benchmarks, exemplified by the HELM (Classic) leaderboards\footref{footnote:HELM (Classic)}. This method ensures consistency and reliability in evaluation standards.
% \item \textit{Submission of prediction files}: Participants submit their prediction results, obtained through the provided API, for evaluation against the reference results. This approach is exemplified by the leaderboards hosted at the Allen Institute for AI\footnote{\url{https://leaderboard.allenai.org}\label{footnote:Allen Institute for AI}}, which promote participation and diversity in submissions.
% \item \textit{Uploading prediction results}: Participants submit their prediction results derived from the test dataset provided for comparison with reference results, as seen in LLMEval\footnote{\url{https://github.com/llmeval}\label{footnote:LLMEval}}.
% \item \textit{API or model submission for evaluation}: Participants provide their models or inference APIs for direct evaluation by leaderboard administrators against reference results, a practice illustrated by the . This allows for a thorough and unbiased assessment of the models.
% \item \textit{Competitive arena through crowd evaluation}: Participants submit their models or inference APIs to be included in a competitive arena, such as Chatbot Arena\footnote{\url{https://chat.lmsys.org}\label{footnote:Chatbot Arena}}, where the audience evaluates the submissions compared to each other. This method leverages crowd wisdom for a more dynamic and interactive evaluation process.
% \end{itemize}
% Each of these methodologies offers unique advantages and challenges that contribute to comprehensive and multifaceted leaderboard submission practices. Once the evaluation results are obtained, it is incumbent on the leaderboard administrators to meticulously organize these results according to specific strategies. This process culminates in the formation of ``candidate leaderboards'', preliminary versions that are not yet ready for public release. Once all evaluations are complete and certain criteria have been met, these candidate leaderboards are published on specific host platforms, such as GitHub. Over time, these leaderboards may undergo iterations, leading to the creation of different published versions. Subsequent versions retire the previous ones, which are so-called ``deprecated leaderboards''. Additionally, we actively seek community feedback at regular intervals to inform future improvements to the leaderboards. This feedback can come from discussions on the hosting platforms' communication channels or through expert publications in the field. At any point in the lifecycle, a retrospective analysis or review mechanism may be introduced. This approach ensures the leaderboards' accuracy and relevance, incorporating the latest data and continuous enhancements influenced by the community feedback. 

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{figures/rq1/Leaderboard-Operations.pdf}
% \caption{The core leaderboard operations.}
% \label{fig:leaderboard operations}
% \centering
% \end{figure}

    % \item \textbf{Administrator}: The entity that publish and maintain the leaderboards.
    % \item \textbf{Evaluator}: The entity that performs the evaluation, which can be a human or an LLM.
    % \item \textbf{Collector}: The entity that collects the evaluation from specified submission venues, which can be a human or a scraper.

 %This gap in the literature represents an untapped opportunity for investigation. % we observe a notable trend among leaderboard publishers: the segmentation of evaluation records into more granular and manageable subdivisions, rather than consolidating all data into a single, overarching leaderboard. We refer to these subdivisions as ``leaderboard splits'' throughout our study. In contrast, we term those leaderboards with multiple splits as ``multi-split leaderboards''  throughout our study. This practice allows for a more nuanced understanding and comparison of model performance across different facets of a problem domain. Thus, we summarize the organization strategies from the collected leaderboards and find there are $20$ organization strategies adopted by different leaderboard publishers. Table~\ref{tab:oraganization strategy} summarizes the $19$ oraganization strategies, .

% This nuanced approach not only enhances the granularity of model evaluation, but also promotes a more segmented and thorough analysis of model performance across diverse scenarios.


% We investigate strategies for oraganization leaderboards, with particular emphasis on the techniques used by publishers to divide evaluation results into smaller and more manageable segments, known as ``leaderboard splits''. This approach aims to efficiently handle the increasing volume of data generated from evaluations, facilitating simpler analysis and comparison. 

% First, we begin with a leaderboard list and a benchmark list to include all the leaderboards and benchmarks identified in the collected literature, respectively. Next, we iterate two lists in an alternate manner to collect the rest of the leaderboards as follows. For each leaderboard in the leaderboard list, we first add the supported benchmarks to the benchmark list if the benchmark does not exist. We then examine the leaderboard documentation for any other mentioned leaderboards and add them to the leaderboard list if the leaderboard does not exist. For each benchmark in the benchmark list, we search the benchmark on Google for its provenance, so that we check if any leaderboards exist on this particular benchmark. If so, we add the new leaderboards to the leaderboard list if it has not been examined previously. This process is done iteratively and complete when all the leaderboard and their supported benchmarks are examined. 

% \item In particular, our selection of leaderboards is based on their constituent benchmarks, rather than on their names. This distinction is important because leaderboards that share identical names can encompass entirely different sets of benchmarks. An illustrative example is the two OpenEval leaderboards\footnote{\url{https://github.com/NTDXYG/open-eval}}\footnote{\url{http://openeval.org.cn}}, which, despite sharing the same name, comprise completely distinct benchmarks. 

% \zhimin{this paragraph explain the structured evaluation literature}
% \paragraph{Automation and structured evaluation}: The emergence of automated systems for the extraction and management of leaderboard data is a crucial development to address the scalability and efficiency of benchmarking efforts. TELIN~\cite{yang2022telin} introduces a multi-modal framework designed to automate the extraction of leaderboard data from scientific publications, a concept that resonates with our exploration of LBOps. By mitigating manual effort and streamlining the leaderboard update process, TELIN shares our goal of improving the operational efficiency of FM leaderboards. Similarly, Kabongo~et~al.~\cite{kabongo2021automated,kabongo2023orkg} present innovative approaches to automate the generation of leaderboards and their integration into digital libraries and knowledge graphs. These efforts underscore the importance of systematic organization and accessibility of leaderboard information, themes central to our investigation of the structural aspects of FM leaderboards.

% hosted on platforms other than Papers~With~Code. The rationale behind this exclusion lies in the collaborative and crowd-sourced nature of leaderboards on Papers~With~Code, which diverges from the administrator-driven mechanisms typically observed. 

% \zhimin{this paragraph explain the enhanced evaluation platforms literature}
% \paragraph{Enhanced evaluation platforms}: Dynaboard~\cite{ma2021dynaboard} represents a significant step towards addressing reproducibility, accessibility, and a wider scope of evaluation in evaluations of the NLP model. By allowing the collection of additional metrics beyond performance, such as memory use and robustness, Dynaboard aligns with our call for a more structured and comprehensive evaluation of FM performance. The approach to standardizing evaluations offers valuable insight into the focus of our study on operational improvements and benchmarking methodologies. Rodriguez~et~al.~\cite{rodriguez2021evaluation} propose a Bayesian leaderboard model to overcome traditional evaluation limitations, further complementing our research. Their work on guiding annotation and identifying errors mirrors our interest in refining the evaluation processes within FM leaderboards, highlighting the potential for innovative methodologies to address current shortcomings.

% \zhimin{this paragraph explain the evaluation frameworks and metrics literature}
% \paragraph{Evaluation frameworks \& metrics}: Mishra~et~al.~\cite{mishra2021robust} introduce alternate metrics and a visual analytics tool to customize leaderboards. This perspective on minimizing performance inflation and facilitating fair model evaluations intersects with our study's exploration of structuring strategies and the challenges in managing LBOps effectively. Explainaboard~\cite{liu2021explainaboard} provides a comprehensive evaluation framework that enhances the utility of traditional leaderboards by offering in-depth analysis methods. This work's emphasis on broad task and language coverage parallels our initiative to uncover insights into the operational dynamics and organizational structures of FM leaderboards, advocating for a more nuanced understanding and application of evaluation practices.

% \zhimin{why our study is unique compared with the above}
% Our study aims to bridge the literature gap by focusing on the operational dynamics, organizational structures, and the challenges inherent in managing FM leaderboards. Drawing inspiration from and building on the foundations laid by the related work discussed, we seek to contribute valuable knowledge to the field, guiding future improvements in FM benchmarking and leaderboard operations (LBOps).

% This misalignment significantly hinders readability and usability, detracting from the overall effectiveness of the benchmark. 
% UML offers a powerful toolkit for depicting system architectures, making it an ideal choice for visualizing the components and relationships within a leaderboard system.
% The Open LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}} and its counterpart\footnote{\url{https://huggingface.co/spaces/gsaivinay/open_llm_leaderboard}} differ minimally, adding only two submissions for GPT-3.5 and GPT-4. 

    % \toprule
    % $S_{\usestrategyIndex}$ \textbf{\#Multiple Choice Options} \\ 
    % \midrule
    % \textbf{Definition}: This strategy pertains to the structuring of leaderboards based on the number of options provided in the multiple choice questions. \\
    % \textbf{Example}: HELM~\cite{bommasani2023holistic} (Classic) serves as a comprehensive benchmark for evaluating language models in a wide range of scenarios and metrics. It organizes several of its leaderboards within the ``Vary Multiple-choice Strategy'' group, each featuring a different range of options. \\
    % \\
    
% \subsubsection{Retirement}

% \zhimin{this section discusses retirement operations in terms of 8 dimensions}
% We find that retirement occurs in $6$ dimensions, including models, datasets, records, reports, submissions, and leaderboards. 
% \begin{itemize}
%     \item \textit{Evaluated Model}: In HELM (Classic)~\cite{bommasani2023holistic}, models highlighted in gray, such as ``OpenAI/text-davinci-001''\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}, are considered deprecated.
%     \item \textit{Evaluation Dataset}: Although the original HELM publication~\cite{bommasani2023holistic} includes WikiText-103~\cite{merity2016pointer} and NewsQA~\cite{trischler2016newsqa} in its supported scenarios, these benchmarks are not available for evaluation on current leaderboards\footnote{\url{https://github.com/stanford-crfm/helm/issues/2239}}. Furthermore, the DROP~\cite{dua2019drop} benchmark was removed from the Open LLM Leaderboard due to unexpected problems in scoring and normalization\footnote{\url{https://huggingface.co/blog/leaderboard-drop-dive}}. Similarly, the ``junior-dev'' dataset is deprecated in the CanAiCode Leaderboard\footnote{\url{https://huggingface.co/spaces/mike-ravkine/can-ai-code-results/discussions/7}}.
%     \item \textit{Evaluation Record}: CanAiCode Leaderboard\footnote{\url{https://huggingface.co/spaces/mike-ravkine/can-ai-code-results}\label{footnote:CanAiCode Leaderboard}} previously displayed results from the deprecated benchmark ``junior-v1''\footnote{\url{https://huggingface.co/spaces/mike-ravkine/can-ai-code-results/discussions/3}}. Furthermore, several leaderboards, such as C-Eval\footnote{\url{https://github.com/hkust-nlp/ceval/issues/76}}, LAiW\footnote{\url{https://huggingface.co/spaces/daishen/SCULAiW/discussions/1}}, Xiezhi\footnote{\url{https://github.com/MikeGu721/XiezhiBenchmark/issues/6}}, and L-Eval\footnote{\url{https://github.com/OpenLMLab/LEval/issues/10}}, face issues of desynchronization with their latest evaluation results.
%     \item \textit{Evaluation Report}: PromptBench has been significantly updated since its first version~\cite{zhu2023promptbench1}, now incorporating DyVal~\cite{zhu2023dyval} and prompt engineering benchmarks~\cite{zhu2023promptbench2}, rendering the initial report obsolete\footnote{\url{https://github.com/microsoft/promptbench/issues/52}}\footnote{\url{https://github.com/microsoft/promptbench/issues/50}}.
%     \item \textit{Evaluation Submission}: The ANLI~\cite{nie2019adversarial} GitHub repository is archived, making its submission guideline deprecated\footnote{\url{https://github.com/facebookresearch/anli}}. Similarly, the RAFT leaderboard\footnote{\url{https://huggingface.co/spaces/ought/raft-leaderboard}} suspends new submissions due to maintenance, and the Spider leaderboard\footnote{\url{https://yale-lily.github.io/spider}} has halted new submissions in anticipation of Spider 2.0's release.
%     \item \textit{Leaderboard}: LLMEval\footnote{\url{http://llmeval.com}} now exclusively adopts the most recent benchmark, LLMEval-3\footnote{\url{https://github.com/llmeval/llmeval-3}}, for model evaluation. This update renders its predecessors, LLMEval-1\footnote{\url{https://github.com/llmeval/llmeval-1}} and LLMEval-2\footnote{\url{https://github.com/llmeval/llmeval-2}}, obsolete.
% \end{itemize}


% We identify and differentiate four core evaluation practices within the development lifecycle of the leaderboard, as delineated in Figure~\ref{fig:evaluation practices}. These practices are categorized into two main groups: strategies to generate evaluation results and methodologies to submit artifacts to leaderboards. The initial group focuses on obtaining the evaluation results. Specifically:
% \begin{itemize}
%     \item Subfigure (a) illustrates the process of model evaluation, where a model undergoes evaluation against a specified benchmark to produce corresponding results.
%     \item Subfigure (b) describes a method by which users can directly access evaluation results from existing multivocal literature, such as articles, blogs, and reports. This approach is predominantly observed in PapersWithCode, with only a few exceptions found elsewhere, notably LLM-Leaderboard\footnote{\url{https://github.com/LudwigStumpp/llm-leaderboard}} and SuperCLUE-Math6\footnote{\url{https://github.com/CLUEbenchmark/SuperCLUE-Math6}}.
% \end{itemize}
% The second group pertains to the submission of artifacts to leaderboards:
% \begin{itemize}
%     \item Subfigure (c) details a self-evaluating submission process, where submitters provide their evaluation results for review by leaderboard maintainers.
%     \item Subfigure (d) covers the third-party evaluating submission approach. Here, the authors provide either the model repository or an inference API following the submission guidelines. The leaderboard maintainers then conduct the evaluation using the provided model or API.
% \end{itemize}

%This obsolescence can arise from various factors, such as the evolution of benchmarks, changes in evaluation criteria, or infrequent updates, leading to a mismatch with the latest evaluation results. 

% Furthermore, our analysis extends to examining the context of each pattern, focusing on both its occurrence and the feasibility of implementing solutions. This exploration has culminated in the formulation of two pivotal questions concerning the patterns.

% We also evaluate the context of each pattern, both in terms of where it is observed and where potential solutions could be implemented. This analysis led us to propose two key questions related to the patterns.
% \begin{itemize}
%     \item Originality: How readily can one pinpoint each pattern based on its source? Potential sources include: (a) leaderboard, (b) documentation, (c) academic paper, (d) technical report, (e) community interaction, such as issue trackers, and (f) source code.
%     \item Solvability: How difficult is it to address each pattern based on available means?
% \end{itemize}
% These questions aim to evaluate the originality and solvability of the patterns across various sources. 

% \subsection{Prevalence Ranking}
% \textbf{Question:} How popular are the leaderboards published in different sources?
% \textbf{Conclusion:} Regarding prevalence, PapersWithCode emerges as the most prominent platform for publishing leaderboards, followed by GitHub, independently hosted websites, HuggingFace, and AI2, in descending order.

% \subsection{Provision Ranking}
% \textbf{Question:} How difficult is it for users to provision new leaderboards from different sources?

    % \toprule
    % $P_{\useIndex}$ \textbf{Idle Entity} \\ 
    % \midrule
    % \textbf{Type}: \textit{Issue} \\
    % \textbf{Category}: \textit{Leaderboard} \\
    % \textbf{Definition}: This pattern identifies leaderboards that are not available to the public. \\
    % \textbf{Example}:  \\
    % \\


% , and MIND\footnote{\url{https://msnews.github.io/\#leaderboard}}

% We ignore leaderboards primarily centered on team performance, such as  These platforms prioritize participant results rather than explicitly showcasing model capabilities, making it unclear whether they include foundation models. 
% Additionally, leaderboards hosted on personal websites, for example, TextSynth Server\footnote{\url{https://bellard.org/ts_server}}, are omitted because they do not allow new submissions. 

    
    % \toprule
    % $P_{\useIndex}$ \textbf{Graphical Entity} \\ 
    % \midrule
    % \textbf{Type}: \textit{Heterogeneity} \\
    % \textbf{Category}: \textit{Leaderboard} \\
    % \textbf{Definition}: This pattern identifies leaderboards that are presented in a chart format rather than in a traditional table format. \\
    % \textbf{Example}: Notable examples include LMExamQA~\cite{bai2023benchmarking}\footnote{\url{https://lmexam.com}}, MMVP~\cite{tong2024eyes}\footnote{\url{https://github.com/tsb0601/MMVP}}, Xiezhi~\cite{gu2023xiezhi}\footnote{\url{https://github.com/MikeGu721/XiezhiBenchmark}}, and TouchStone~\cite{bai2023touchstone}\footnote{\url{https://github.com/ofa-sys/touchstone}}, which present their leaderboards as charts. In contrast, SafetyBench~\cite{zhang2023safetybench}\footnote{\url{https://github.com/thu-coai/SafetyBench}}, LawBench~\cite{fei2023lawbench}\footnote{\url{https://lawbench.opencompass.org.cn/leaderboard}}, and LAiW~\cite{dai2023laiw}\footnote{\url{https://huggingface.co/spaces/daishen/SCULAiW}} utilize a dual format, showcasing their leaderboards both as tables and as charts.\\
    % \\



    % \\
    % \toprule
    % $P_{\useIndex}$ \textbf{Undownloadable Entity} \\ 
    % \midrule
    % \textbf{Type}: \textit{Heterogeneity} \\
    % \textbf{Category}: \textit{Leaderboard} \\
    % \textbf{Definition}: This pattern identifies leaderboards that do not provide an easy means to download the evaluation records. \\
    % \textbf{Example}: Currently, many leaderboards, including those on PapersWithCode and various independent platforms, lack the functionality to export evaluation results in formats such as CSV. This absence hinders users from performing rigorous or systematic comparisons across different leaderboards. As a workaround, users often resort to developing custom scraping scripts to extract these evaluation records. Alternatively, they may employ a rudimentary comparison method, relying on visual inspection of the results. However, this approach is less precise and more time-consuming. \\
    % \bottomrule
    
    % \toprule
    % $P_{\useIndex}$ \textbf{Suspended Entity} \\ 
    % \midrule
    % \textbf{Type}: \textit{Issue} \\
    % \textbf{Category}: \textit{Leaderboard} \\
    % \textbf{Definition}: This pattern pertains to leaderboards that currently do not accept new evaluation records. \\
    % \textbf{Example}:  \\
    % \\

% \textbf{Findings:}
% \begin{itemize}
% \item \textbf{AI2:} Leaderboard provision is not supported.
% \item \textbf{GitHub:} It provides customization of leaderboards through markdown, subject to certain limitations.
% \item \textbf{HuggingFace:} Leaderboard provision is available within the confines of HuggingFace Spaces features.
% \item \textbf{PapersWithCode:} It supports the creation of new leaderboards, which require adhesion to a set template. Mandatory fields include ``Rank'', ``Model'', ``Paper'', ``Code'', ``Result'', ``Year'', and ``Tags''. Users have the discretion to fill these fields and can only customize the evaluation metrics. PapersWithCode is largely community-contributed - anyone can add a benchmarking result or a task, provided the benchmarking result is publicly available in a pre-print repository, conference proceeding, or journal. 
% \item \textbf{independently hosted websites:} Users have the maximum customization freedom to create new leaderboards.
% \end{itemize}

% \textbf{Conclusion:} Regarding the provision of leaderboards, independently hosted websites offer the greatest flexibility. HuggingFace Spaces rank next due to their supportive resources and tools for deploying and sharing interactive leaderboards. GitHub follows, offering moderate customization capabilities. PapersWithCode has more restrictive templates, and AI2 ranks last, not allowing user-created leaderboards.

% \subsection{Submission Ranking}
% \textbf{Question:} How flexible are the options available to users to submit evaluation records to various sources?

% \textbf{Findings:}
% \begin{itemize}
% \item \textbf{AI2:} Submissions here require adherence to specific instructions and format, with users expected to submit their evaluation results directly.
% \item \textbf{GitHub:} This platform also requires users to follow a set of instructions and formats, but submissions are made through a pull request.
% \item \textbf{HuggingFace:} Adopting a method similar to GitHub, HuggingFace allows submissions via a pull request or through a specific procedure to upload models that are yet to be evaluated.
% \item \textbf{PapersWithCode:} The flexibility here varies depending on the type of leaderboard being used. There are two main types: the ``crowdsourced leaderboard'', curated by PapersWithCode crowdworkers, and the ``community leaderboard'', curated by HuggingFace repository owners of evaluated models. The crowdsourced leaderboard allows open submission of self-reported metrics or predictions of the corresponding datasets, while the community leaderboard restricts changes to those directly involved with the evaluated models.
% \item \textbf{independently hosted websites:} These sources are similar to AI2 in that they require users to follow specific instructions and formats for direct submission of evaluation results.
% \end{itemize}

% \textbf{Conclusion:} Regarding submission flexibility, PapersWithCode stands out as the most accommodating. HuggingFace, AI2, GitHub, and independently hosted websites offer relatively similar levels of flexibility.

% \subsection{Transparency Ranking}
% \textbf{Question:} How transparent are the evaluation records from different sources?

% First of all, always try to be transparent about what you have done and what you have discovered, as this will make it easier for other people to build on your work. In particular, it is good practice to share your models in an accessible way. For example, if you used a script to implement all your experiments, then share the script when you publish the results. This means that other people can easily repeat your experiments, adding confidence to your work. It also makes it much easier for people to compare models, since they no longer have to reimplement everything from scratch in order to ensure a fair comparison. Knowing that you will be sharing your work also encourages you to be more careful, document your experiments well, and write clean code, which benefits you as much as anyone else. It is also worth noting that issues surrounding reproducibility are gaining prominence in the ML community, so in the future you may not be able to publish work unless your workfow is adequately documented and shared.

% \textbf{Findings:}
% \begin{itemize}
% \item \textbf{AI2:} Users can access the submission detail page by clicking on a evaluation record. This page displays the creation date, publication date, description of the evaluated model, and contributor's details.
% \item \textbf{GitHub:} The inclusion of provenance links varies by the leaderboard design. Among the 77 publisher-based leaderboards examined on GitHub, only 35.06\% (27) provide provenance links to their evaluation records.
% \item \textbf{HuggingFace:} Similar to GitHub, the attachment of provenance links is at the discretion of the leaderboard designers. In our study of 21 publisher-based leaderboards on HuggingFace, 66.67\% (14) included provenance links.
% \item \textbf{PapersWithCode:} On crowdsourced leaderboards, evaluation records typically include links to the original paper, the GitHub repository, and the specific tables of the original paper where the evaluation originates. A comprehensive examination of $6,735$ evaluation records from these leaderboards reveals that a significant majority $92.65\%$ ($6,240$ records) contain links to associated papers, while 85.48\% (5,334 records) are linked to GitHub repositories. In particular, the average frequency of attachment of papers to the GitHub repository is $98.94\%$, and for GitHub repository links it is $90.17\%$. This high incidence of link inclusion underscores the extensive coverage of platform provenance on crowdsourced leaderboards. In contrast, community leaderboards only provide links to the model repositories on HuggingFace, with the evaluation records themselves being located within these repositories.
% \item \textbf{independently hosted websites:} The practice of including provenance links also varies among independently hosted websites. In our analysis of $43$ publisher-based leaderboards, only $23.26\%$ ($10$) included provenance links.
% \end{itemize}

% \textbf{Conclusion:} Regarding transparency, PapersWithCode leads, exhibiting a high level of detail in its provenance links, closely followed by AI2. HuggingFace provides a moderate level of provenance information. GitHub offers even less comprehensive details. Finally, independently hosted websites exhibit the least thorough practices in the provision of provenance details within their leaderboards. 

% \subsection{Feedback Ranking}
% \textbf{Question:} How easy is it to provide feedback to the leaderboard maintainers from different sources?

% \textbf{Findings:}
% \begin{itemize}
% \item \textbf{AI2 and PapersWithCode:} Feedback is limited to email communication with the website maintainers.
% \item \textbf{GitHub and HuggingFace:} These platforms offer dual channels of feedback, so users have the option of raising issues or sending emails to the repository maintainers.
% \item \textbf{independently hosted websites:} A majority, 81.40\% (35 out of 43) include a link to their GitHub repository, inviting users to report issues there. Furthermore, almost all, 97. 67\% (42 out of 43), provide contact information for direct communication, with OpenEval\footnote{\url{http://openeval.org.cn/}} being the sole exception.
% \end{itemize}

% \textbf{Conclusion:} Regarding ease of feedback, GitHub and HuggingFace emerge as the most accessible, offering multiple feedback mechanisms. They are closely followed by independently hosted websites, which predominantly support issue reporting through GitHub and direct contact. However, AI2 and PapersWithCode present more limited options, relying primarily on email communication for feedback.

% \subsection{Review Ranking}
% \textbf{Question:} How strict is the review for new submissions from different sources? 

% \textbf{Findings:}
% \begin{itemize}
%     \item \textbf{AI2, GitHub, HuggingFace, independently hosted websites:} For these sources, the inclusion of submissions on the leaderboard is contingent upon a review process conducted by the leaderboard maintainers.
%     \item \textbf{PapersWithCode:} Unlike the other sources, PapersWithCode implements a loose review process for evaluation records\footnote{This is confirmed by the email with PapersWithCode maintainers}, regardless of whether they come from contributors or community leaderboards.
% \end{itemize}

% \textbf{Conclusion:} Regarding review strictness, AI2, GitHub, HuggingFace, and independently hosted websites all employ a review process by their respective leaderboard maintainers to determine the inclusion of new submissions. PapersWithCode stands out for its relatively lenient review process for evaluation records, applicable to both contributor and community leaderboards.

%Our focus is on whether the constituent benchmark remains unchanged. For example, Ko-HellaSwag on the Open Ko-LLM Leaderboard\footnote{\url{https://huggingface.co/spaces/upstage/open-ko-llm-leaderboard}} is treated as a variant of HellaSwag~\cite{zellers2019hellaswag} but not as HellaSwag itself. 

% \textbf{Example}: EvalPlus~\cite{liu2023your}\footnote{\url{https://evalplus.github.io/leaderboard.html}} maintains two different leaderboards for HumanEval~\cite{chen2021evaluating} and MBPP~\cite{austin2021program}. Additionally, it features an aggregated leaderboard that computes the average scores from the two aforementioned leaderboards.

% \subsection{Leaderboard Representation}

% Due to the significant diversity among the leaderboards we collected, we represent them using different organization standards, as illustrated in Figure~\ref{fig:leaderboard representation}.

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{figures/rq1/Leaderboard Organization.pdf}
% \caption{Leaderboard hierarchy based on different representation.}
% \label{fig:leaderboard representation}
% \centering
% \end{figure}

% \item \textbf{Publisher-based Leaderboards:} Leaderboards released by the same group of publishers are grouped under this criterion. For example, the LLM-Leaderboard\footnote{\url{https://github.com/LudwigStumpp/llm-leaderboard}}, available on GitHub, HuggingFace\footnote{\url{https://huggingface.co/spaces/ludwigstumpp/llm-leaderboard}}, and an independent platform\footnote{\url{https://llm-leaderboard.streamlit.app}}, is considered a single entity. Our dataset comprises $544$ publisher-based leaderboards in total.
% \item \textbf{Template-based Leaderboards:} Publisher-based leaderboards on certain platforms (\eg AI2 and PapersWithCode) that adhere to specific templates are called ``template-based leaderboards.'' Those not following any template are referred to as ``custom leaderboards'' in our study.
% In our study, we define a ``scenario'' as a specific set of conditions crafted to examine various facets of a model's performance. This variability often leads to the segmentation of a single comprehensive leaderboard into several specialized sub-leaderboards, each focusing on distinct performance aspects.
